Blue Straggler Stars: Early Observations that Failed to Solve the Problem

In this chapter, I describe early ideas on blue stragglers, and various observations (some published, some not) that promised but failed to resolve the question of their origin. I review the data and ideas that were circulating from Allan Sandage's original discovery in 1953 of "anomalous blue stars" in the globular cluster M3, up until about 1992, when what seems to have been the only previous meeting devoted to Blue Straggler Stars (BSSs) was held at the Space Telescope Science Institute.

==> common.tex <==
% Bibliography and bibfile
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull. astr. Inst. Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron. Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J. Astron. Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jcap{J. Cosmology Astropart. Phys.}%
          % Journal of Cosmology and Astroparticle Physics
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%
          % Physical Review C
\def\prd{Phys.~Rev.~D}%
          % Physical Review D
\def\pre{Phys.~Rev.~E}%
          % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.~Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\def\physrep{Phys.~Rep.}%
          % Physics Reports
\def\physscr{Phys.~Scr}%
          % Physica Scripta
\def\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

\newcommand{\gras}[1]{\mbox{\boldmath $#1$}}
\def\arcsec{\hbox{$^{\hbox{\rlap{\hbox{\lower4pt\hbox{$\,\prime\prime$}}          }\hbox{$\frown$}}}$}}
\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\gtsima{$\; \buildrel > \over \sim \;$}
\def\lsim{\lower.5ex\hbox{\ltsima}}
\def\gsim{\lower.5ex\hbox{\gtsima}}
\def\lapp{\ifmmode\stackrel{<}{_{\sim}}\else$\stackrel{<}{_{\sim}}$\fi}
\def\gapp{\ifmmode\stackrel{>}{_{\sim}}\else$\stackrel{<}{_{\sim}}$\fi}

\def\msol{\,\mathrm{M}_\odot}
\def\media#1{\langle #1\rangle}
\def\kms{~{\rm km~ s}^{-1}}
\def\sigp{\sigma_{\rm P}}


\def\aapr{A\&A Rev. }
\def\apjl{ApJL }
\def\aj{AJ }
\def\apj{ApJ }
\def\pasp{PASP }
\def\spie{SPIE }
\def\apjs{ApJS }
\def\araa{ARAA }
\def\aap{A\&A }
\def\mnras{MNRAS }
\def\nat{Nature }

\newcommand{\lesssim}    {\mbox{\rlap{\hbox{\lower3pt\hbox{\ensuremath{\sim}}}}\raise1.5pt\hbox{\ensuremath{<}}}}%
\newcommand{\lsim}       {\lesssim}%
\newcommand{\la}         {\lesssim}% For Springer A&A compliance...
\newcommand{\gtrsim}     {\mbox{\rlap{\hbox{\lower3pt\hbox{\ensuremath{\sim}}}}\raise1.5pt\hbox{\ensuremath{>}}}}%
\newcommand{\gsim}       {\gtrsim}%
\newcommand{\ga}         {\gtrsim}%
\newcommand{\sq}         {\mbox{\rlap{\ensuremath{\sqcap}}\ensuremath{\sqcup}}}%
\newcommand{\arcdeg}     {\mbox{\ensuremath{{}^\circ}}}%
\newcommand{\arcmin}     {\mbox{\ensuremath{{}^\prime}}}%
\newcommand{\arcsec}     {\mbox{\ensuremath{{}^{\prime\prime}}}}%

% Journal abbreviations
\def\aj{\rmfamily{AJ~}}           % Astronomical Journal
\def\apj{\rmfamily{ApJ~}}         % Astrophysical Journal
\def\apjl{\rmfamily{ApJ~}}        % Astrophysical Journal, Letters
\def\apjs{\rmfamily{ApJS~}}       % Astrophysical Journal, Supplement
\let\apjlett=\apjl
\let\apjsupp=\apjs
\def\aap{\rmfamily{A\&A~}}        % Astronomy and Astrophysics
\let\astap=\aap
\def\araa{\rmfamily{ARA\&A~}}     % Annual Review of Astronomy and Astrophysics
\def\aapr{\rmfamily{A\&A~Rev.~}}  % Astronomy and Astrophysics Reviews
\def\aaps{\rmfamily{A\&AS~}}      % Astronomy and Astrophysics, Supplement
\def\mnras{\rmfamily{MNRAS~}}     % Monthly Notices of the Royal Astron. Soc.
\def\pasp{\rmfamily{PASP~}}       % Publications of the Astron. Soc. o/t Pacific
\def\apss{\rmfamily{Ap\&SS~}}     % Astrophysics and Space Science
\def\pasj{\rmfamily{PASJ~}}       % Publications of the Astron. Soc. of Japan
\def\pra{\rmfamily{Phys.~Rev.~A~}}% Physical Review A: Atomic, Molecular, and  
                                  %   Optical Physics
\def\prb{\rmfamily{Phys.~Rev.~B~}}% Physical Review B: Condensed Matter and
                                  %   Materials Physics
\def\prc{\rmfamily{Phys.~Rev.~C~}}% Physical Review C: Nuclear Physics
\def\prd{\rmfamily{Phys.~Rev.~D~}}% Physical Review D: Particles, Fields,
                                  %   Gravitation and Cosmology
\def\pre{\rmfamily{Phys.~Rev.~E~}}% Physical Review E: Statistical, Nonlinear,
                                  %   and Soft Matter Physics
\def\rmp{\rmfamily{Rev.~Mod.~Phys.~}}% Reviews of Modern Physics
\def\prl{\rmfamily{Phys.~Rev.~Lett.~}}% Physical Review Letters
\def\nat{\rmfamily{Nature~}}      % Nature
\def\sci{\rmfamily{Science~}}     % Science
\def\skytel{\rmfamily{S\&T~}}     % Sky and Telescope
\def\ao{\rmfamily{Appl.~Opt.~}}   % Applied Optics
\let\applopt=\ao
\def\azh{\rmfamily{AZh~}}         % Astronomicheskii Zhurnal
\def\baas{\rmfamily{BAAS~}}       % Bulletin of the AAS
\def\jrasc{\rmfamily{JRASC~}}     % Journal of the Royal Astron. Soc. of Canada
\def\memras{\rmfamily{MmRAS~}}    % Memoirs of the Royal Astron. Soc.
\def\qjras{\rmfamily{QJRAS~}}     % Quarterly Journal of the Royal Astron. Soc.
\def\solphys{\rmfamily{Sol.~Phys.~}}% Solar Physics
\def\sovast{\rmfamily{Soviet~Ast.~}}% Soviet Astronomy
\def\ssr{\rmfamily{Space~Sci.~Rev.~}}% Space Science Reviews
\def\zap{\rmfamily{ZAp~}}         % Zeitschrift fuer Astrophysik
\def\iauc{\rmfamily{IAU~Circ.~}}  % IAU Cirulars
\let\iaucirc=\iauc
\def\aplett{\rmfamily{Astrophys.~Lett.~}}% Astrophysics Letters
\def\apspr{\rmfamily{Astrophys.~Space~Phys.~Res.~}}% Astrophysics Space Physics
                                  % Research
\def\bain{\rmfamily{Bull.~Astron.~Inst.~Netherlands~}}% Bulletin of the 
                                  % Astronomical Institute of the Netherlands
\def\fcp{\rmfamily{Fund.~Cosmic~Phys.~}}% Fundamental Cosmic Physics
\def\gca{\rmfamily{Geochim.~Cosmochim.~Acta~}}% Geochimica Cosmochimica Acta
\def\grl{\rmfamily{Geophys.~Res.~Lett.~}}% Geophysics Research Letters
\def\jcp{\rmfamily{J.~Chem.~Phys.~}}% Journal of Chemical Physics
\def\jgr{\rmfamily{J.~Geophys.~Res.~}}% Journal of Geophysics Research
\def\jqsrt{\rmfamily{J.~Quant.~Spec.~Radiat.~Transf.~}} % Journal of Quantitative
                                  % Spectroscopy and Radiative Transfer
\def\memsai{\rmfamily{Mem.~Soc.~Astron.~Italiana~}}
                                  % Mem. Societa Astronomica Italiana
\def\nphysa{\rmfamily{Nucl.~Phys.~A~}}% Nuclear Physics A
\def\physrep{\rmfamily{Phys.~Rep.~}}% Physics Reports
\def\physscr{\rmfamily{Phys.~Scr~}}% Physica Scripta
\def\planss{\rmfamily{Planet.~Space~Sci.~}}% Planetary Space Science
\def\procspie{\rmfamily{Proc.~SPIE~}}% Proceedings of the SPIE
\def\aipconf{\rmfamily{AIP~Conf.~Proc.~}}% AIP Conference Proceedings
\def\aspconf{\rmfamily{ASP~Conf.~Ser.~}}% ASP Conference Series
\def\asslconf{\rmfamily{Ap\&SSL~Conf.~Ser.~}}% ASSL Conference Series}
\def\maps{\rmfamily{MAPS~}}       % Meteoritics and Planetary Science

\usepackage{amsmath}
\usepackage{amssymb}

\def\Teff{$T_{\rm eff}$}
\def\Msun{{\rm M}_\odot}
\def\Rsun{{\rm R}_\odot}
\def\kms{\rm km~s$^{-1}$}

\def\arcsec{\hbox{$^{\hbox{\rlap{\hbox{\lower4pt\hbox{$\,\prime\prime$}}                         }\hbox{$\frown$}}}$}}

\newcommand{\msun}{$M_{\odot}$}
\newcommand{\etal}{{\it et al.}}


\newcommand{\half}{{\ensuremath{\textstyle\frac12}}}
\newcommand{\threehalf}{{\ensuremath{\textstyle\frac32}}}
\newcommand{\third}{{\ensuremath{\textstyle\frac13}}}
\newcommand{\quarter}{{\ensuremath{\textstyle\frac14}}}
\newcommand\apgt{\ {\raise-.5ex\hbox{$\buildrel>\over\sim$}}\ }
\newcommand\aplt{\ {\raise-.5ex\hbox{$\buildrel<\over\sim$}}\ }

\newcommand{\kin}{{\ensuremath K}}
\newcommand{\mbar}{{\ensuremath \langle m\rangle}}
\newcommand{\msun}{{\ensuremath M_\odot}}
\newcommand{\pot}{{\ensuremath U}}
\newcommand{\rvir}{{\ensuremath R_{vir}}}
\newcommand{\rh}{{\ensuremath R_h}}
\newcommand{\rj}{{\ensuremath R_J}}
\newcommand{\rsun}{{\ensuremath R_\odot}}
\newcommand{\tcc}{{\ensuremath t_{cc}}}
\newcommand{\tdis}{{\ensuremath t_{dis}}}
\newcommand{\tdyn}{{\ensuremath t_{dyn}}}
\newcommand{\tr}{{\ensuremath t_r}}
\newcommand{\tenc}{{\ensuremath t_{enc}}}
\newcommand{\trh}{{\ensuremath t_{rh}}}
\newcommand{\trl}{{\ensuremath t_{rl}}}
\newcommand{\tseg}{{\ensuremath t_{seg}}}
\newcommand{\vdisp}{{\ensuremath \langle v^2\rangle}}
\newcommand{\vrms}{{\ensuremath \vdisp^{1/2}}}
\newcommand{\vesc}{{\ensuremath v_{esc}}}
\newcommand{\vinf}{{\ensuremath v_\infty}}

\newcommand{\vv}{{\bf v}}
\newcommand{\vx}{{\bf x}}
\newcommand{\va}{{\bf a}}






==> refbeccari.tex <==
\begin{thebibliography}{99.}%
\bibitem{ca85} Castellani, V.: Astrofisica Stellare. Zanichelli, Bologna (1985) 
\bibitem{ca03} Castellani, V., Degl'Innocenti, S., Marconi, M., Prada Moroni, P.~G., \& Sestito, P.: A\&A \textbf{404}, 645  (2003) 
\bibitem{pi06}  Pietrinferni, Cassisi, Salaris \& Castelli: ApJ \textbf{642}, 797 (2006)
\bibitem{ri00} Richer, H.~B., Hansen, B., Limongi, M., et al.: ApJ \textbf{529}, 318 (2000) 
\bibitem{sa05} Salaris, M., \& Cassisi, S.: Evolution of Stars and Stellar Populations,~Wiley-VCH  (2005)  
\bibitem{sh82} Shu, F.~H.: Journal of the British Astronomical Association \textbf{93}, 45 (1982)
\bibitem{to11} Tognelli, Prada Moroni, Degl'Innocenti: A\& A \textbf{533}, A109 (2011)
\end{thebibliography}


==> refboffin.tex <==
\begin{thebibliography}{99}
\bibitem{Abate13} Abate, C., Pols, O.~R., Izzard, R.~G., Mohamed, S.~S., de Mink, S.~E.: A\&A {\bf 552}, A26  (2013)
\bibitem{Bid81} Bidelman, W. P.: AJ {\bf 86}, 553 (1981)
\bibitem{BK51} Bidelman, W. P., Keenan, P. C.: ApJ {\bf 114}, 473 (1951)
\bibitem{Blind11} Blind, N., Boffin, H.~M.~J., Berger, J.-P., Le Bouquin, J.-B., M{\'e}rand, A., Lazareff, B., Zins, G.: A\&A {\bf 536}, A55 (2011)
\bibitem{BA94} Boffin, H.~M.~J., Anzer, U.: A\&A {\bf 284}, 1026 (1994)
\bibitem{BoMes14} Boffin, H. M. J., Blind, N., Hillen, M., et al.: Messenger {\bf 156} (2014)
\bibitem{BCP93} Boffin, H. M. J., Cerf, N., Paulus, G.: A\&A {\bf 271}, 125 (1993)
\bibitem{Bo14} Boffin, H.~M.~J., Hillen, M., Berger, J.~P., et al.: A\&A {\bf 564}, A1 (2014)
\bibitem{BJ88} Boffin, H.~M.~J., Jorissen, A.: A\&A {\bf 205}, 155 (1988)
\bibitem{BoMi12} Boffin, H.~M.~J.,  Miszalski, B.: in Evolution of Compact Binaries, ASPC {\bf 447}, p. 159 (2011)
\bibitem{Bo12} Boffin, H.~M.~J., Miszalski, B., Rauch, T., et al.: Science {\bf  338}, 773  (2012)
%Science
\bibitem{BPC92} Boffin, H.~M.~J., Paulus, G.,  Cerf, N.: in Binaries as Tracers of Star Formation, Cambridge Univ. Press, p. 26 (1992)
\bibitem{BTJ94} Boffin, H.~M.~J., Theuns, T., Jorissen, A.: MmSAI {\bf 65}, 1199 (1994)
\bibitem{BZ94} Boffin, H.~M.~J., Za{\v c}s, L.: A\&A {\bf 291}, 811 (1994)
\bibitem{BoNP84} B\"ohm-Vitense, E., Nemec, J., Proffitt, C.: ApJ {\bf 278}, 726 (1984)
\bibitem{Bona08} Bona{\v c}i{\'c} Marinovi{\'c}, A.~A., Glebbeek, E., Pols, O.~R.: A\&A {\bf 480}, 797  (2008)
\bibitem{1993IAUS..155..397B} Bond, H.~E., Ciardullo, R., Meakes, M.~G.: in Planetary Nebulae, ASPC {\bf 155}, 397 (1993)
\bibitem{2003AJ....125..260B} Bond, H.~E., Pollacco, D.~L., Webbink, R.~F.: AJ {\bf 125}, 260 (2003)
\bibitem{Bondi52} Bondi, H.:  MNRAS {\bf 114}, 195 (1952)
\bibitem{BH44} Bondi, H., Hoyle, F.: MNRAS {\bf 104}, 273 (1944)
\bibitem{BrookTav93} Brookshaw, L., Tavani, M.: ApJ {\bf 410}, 719 (1993)
\bibitem{Cliffe95} Cliffe, J.~A., Frank, A., Livio, M., Jones, T.~W.: ApJL {\bf 447}, 49 (1995)
\bibitem{c03} Corradi, R.~L.~M.: in Symbiotic Stars Probing Stellar Evolution, ASPC {\bf 303}, 393 (2003)
\bibitem{Cor11} Corradi, R.~L.~M., Sabin, L., Miszalski, B., et al.: MNRAS {\bf 410}, 1349  (2011)
%necklace
\bibitem{DM08} De Marco, O.: PASP {\bf 121}, 316 (2009)
\bibitem{Der09} Dermine, T., Jorissen, A., Siess, L., Frankowski, A: A\& A {\bf 507}, 891 (2009)
\bibitem{2014MNRAS.437.1216D} De Rosa, R.~J., Patience, J., Wilson, P.~A., et al.: MNRAS {\bf 437}, 1216 (2014)
\bibitem{Eggleton83} Eggleton, P.~P.: ApJ {\bf 268}, 368 (1983)
\bibitem{Egg92} Eggleton, P. P.: in Evolutionary Processes in Interacting Binary Stars, IAU Symp. 151, Kluwer Academic Publishers, p. 167 (1992)
\bibitem{2008PhDT.......109F} Frew, D.~J.: Ph.D.~Thesis, Macquarie University  (2008)
\bibitem{Gel09} Geller, A.~M., Mathieu, R.~D., Harris, H.~C., McClure, R.~D.: AJ {\bf 137}, 3743 (2009)
\bibitem{Gray01} Gray, R.~O., McGahee, C.~E., Griffin, R.~E.~M., \& Corbally, C.~J.: AJ {\bf 141}, 160  (2011)
\bibitem{Hachisu99} Hachisu, I., Kato, M., Nomoto, K.: ApJ {\bf 522}, 487  (1999)
\bibitem{HL39} Hoyle, F., Lyttleton, R.A.: Proc. Cam. Phil. Soc. {\bf 35}, 405 (1939)
\bibitem{Huang56} Huang, S.S.: AJ  {\bf 61}, 49 (1956)
\bibitem{Hunt71} Hunt, R.: MNRAS {\bf 154}, 141 (1971)
\bibitem{2006PThPh.116.1069I} Isaka, H., Matsuda, T., Boffin, H.~M.~J.:  PThPh  {\bf 116}, 1069 (2006)
\bibitem{JJ87} Jaschek, C., Jaschek, M.: The classification of stars, Cambridge University Press (1987)
\bibitem{Jaha05} Jahanara, B., Mitsumoto, M., Oka, K., Matsuda, T., Hachisu, I., Boffin, H.~M.~J.: A\&A {\bf 441}, 589 (2005)
\bibitem{1996MNRAS.279..180J} Jeffries, R.~D.,  Stevens, I.~R.: MNRAS {\bf 279}, 180 (1996)
\bibitem{Jorissen03} Jorissen, A.: in Symbiotic Stars Probing Stellar Evolution, ASPC {\bf 303}, 25  (2003)
\bibitem{JB92} Jorissen, A., Boffin, H.~M.~J.: in Binaries as tracers of stellar formation, Cambridge Univ. Press, p. 110 (1992)
\bibitem{JoM92} Jorissen, A., Mayor, M.: A\&A {\bf 260}, 115 (1992)
\bibitem{Jo95} Jorissen, A., Hennen, O., Mayor, M., Bruch, A., Sterken, C.: A\&A {\bf 301}, 707 (1995)
%HD165141
\bibitem{Jo98} Jorissen, A., Van Eck, S., Mayor, M., Udry, S.:  A\&A {\bf 332}, 877  (1998)
%orbits of S stars
\bibitem{2005A&A...441.1135J} Jorissen, A., Za{\v c}s, L., Udry, S., Lindgren, H., Musaev, F.~A.: A\&A {\bf 441}, 1135 (2005)
\bibitem{KTL00} Karakas, A.~I., Tout, C.~A., \& Lattanzio, J.~C.: MNRAS {\bf 316}, 689 (2000)
\bibitem{bofko55} Kopal, Z.: Ann. Astrophys.\textbf{18}, 379 (1955)
\bibitem{ko59} Kopal, Z.:  Close binary systems, The International Astrophysics Series, Chapman \& Hall (1959)
\bibitem{La85} Lambert, D. L.: in Cool Stars with Excesses of Heavy-elements, p. 191 (1985)
\bibitem{Lu91} L\"u, P. K.: AJ {\bf 101}, 2229 (1991)
\bibitem{Matsuda87} Matsuda, T., Inoue, M., Sawada, K.: MNRAS  {\bf 226}, 785 (1987)
\bibitem{Matsuda92} Matsuda, T., Ishii, T., Sekino, N., Sawada, K., Shima, E., Livio, M.,
Anzer, U.: MNRAS {\bf 255}, 183 (1992)
\bibitem{Maercker12} Maercker, M., Mohamed, S., Vlemmings, W.~H.~T., et al.: Nature {\bf 490}, 232 (2012)
\bibitem{McFN83} McClure, R. D., Fletcher, J. M., Nemec, J. M.: ApJL {\bf 238}, 35 (1983)
\bibitem{McW90} McClure, R. D., Woodsworth, A. W.: ApJ {\bf 352}, 709 (1990)
\bibitem{Merm} Mermilliod, J.-C., Andersen, J., Latham, D.~W., Mayor, M.: A\&A {\bf 473}, 829  (2007)
\bibitem{Mik07} Mikolajewska, J.: Baltic Astronomy {\bf 16}, 1 (2007)
\bibitem{Mitchell07} Mitchell, D.~L., 
Pollacco, D., O'Brien, T.~J., et al.: MNRAS {\bf 374}, 1404 (2007)
\bibitem{Mis09} Miszalski, B., Acker, A., Moffat, A.~F.~J., Parker, Q.~A., \& Udalski, A.: A\&A {\bf 496}, 813  (2009)
\bibitem{Mis11} Miszalski, B., Jones, D., Rodr{\'{\i}}guez-Gil, P., et al.: A\&A {\bf 531}, A158 (2011)
% jets
\bibitem{2012MNRAS.419...39M} Miszalski, B., Boffin, H.~M.~J., Frew, D.~J., Acker, A., K{\"o}ppen, J., Moffat, A.~F.~J., Parker, Q.~A.: MNRAS {\bf 419}, 39 (2012)
\bibitem{Hen239} Miszalski, B., Boffin, H.~M.~J., Jones, D., et al.: MNRAS {\bf 436}, 3068  (2013)
%Hen2-39
\bibitem{2013MNRAS.428L..39M} Miszalski, B., Boffin, H.~M.~J., Corradi, R.~L.~M.: MNRAS {\bf 428}, L39 (2013)
%Necklace
\bibitem{Sahaietal2006} Morris, M., Sahai, R., Matthews, K., et al.: in Planetary Nebulae in our Galaxy and Beyond, ASPC {\bf 234}, p. 469 (2006)
%AFL3068
\bibitem{Nagae04} Nagae, T., Oka, K., Matsuda, T., Fujiwara, H., Hachisu, I., Boffin, H.~M.~J.: A\&A {\bf 419}, 335 (2004)
\bibitem{Packett81} Packett, W.: A\&A {\bf 102}, 17 (1981)
\bibitem{pacz71} Paczy{\'n}ski, B.: ARA\&A {\bf 9}, 183 (1971)
\bibitem{Passy12} Passy, J.-C., De Marco, O., Fryer, C.~L., et al.: ApJ {\bf 744}, 52 
 (2012)
\bibitem{PlavecKratochvil64} Plavec, M., Kratochvil, P.: Bulletin of the Astronomical Institutes of Czechoslovakia {\bf 15,} 165 (1964)
\bibitem{PM07}  Podsiadlowski, P., Mohamed, S.\ 2007, Baltic Astronomy {\bf 16}, 26 (2007)
\bibitem{Raga09}  Raga, A.~C., Esquivel, A., Vel{\'a}zquez, P.~F., et al.: ApJL {\bf 707}, L6 
 (2009)
\bibitem{bofRaghavan2010}  Raghavan, D.,  McAlister, H. A.,  Henry, T. J., et al.: ApJS {\bf 190}, 1 (2010)
\bibitem{RT12} Ricker, P.~M., Taam, R.~E.: ApJ {\bf 746}, 74 (2012)
\bibitem{Ruffert94} Ruffert, M.: ApJ {\bf 427}, 342 (1994)
\bibitem{Schu72} Schuerman, D.~W.: Ap\&SS {\bf 19}, 351  (1972)
\bibitem{Shima98} Shima, E., Matsuda, T., Anzer, U., Boerner, G., Boffin, H.~M.~J.: A\&A {\bf 337}, 311 (1998)
\bibitem{TBJ96} Theuns, T., Boffin, H.~M.~J., Jorissen, A.: MNRAS {\bf 280}, 1264 (1996)
\bibitem{TJ93} Theuns, T. \& Jorissen, A.: MNRAS {\bf 265}, 946 (1993)
\bibitem{TE88}  Tout, C. A. \& Eggleton, P. P.: MNRAS {\bf 231}, 823 (1988)
\bibitem{Ty13} Tyndall, A.~A., Jones, D., Boffin, H.~M.~J., et al.: MNRAS {\bf 436}, 2082 (2013)
\bibitem{vW14} Van Winckel, H., Jorissen, A., Exter, K., et al.: A\&A {\bf 563}, L10  (2014)
\bibitem{Wa74} Warner, B.: MNRAS {\bf 129}, 263 (1974)
\bibitem{We86} Webbink, R. F.: in Critical Observations vs. Physical Models for Close Binary Systems, Gordon and Breach Science Publishers, p. 403 (1988)
\end{thebibliography}

==> refdavies.tex <==
\begin{thebibliography}{99}

\bibitem{Bacon96}
Bacon, D., Sigurdsson, S.,  Davies, M. B.:  MNRAS {\bf 281}, 830 (1996)

\bibitem{davBH87}
Benz, W. ,  Hills, J. G.:  ApJ {\bf 323}, 614 (1987)

\bibitem{davBH92}
Benz, W. ,  Hills, J. G.:  ApJ {\bf 389}, 546 (1992)

\bibitem{Carney01}
Carney, B. W., Latham, D. W., Laird, J. B., Grant, C. E.,  Morse, J. A.: AJ {\bf 122}, 3419 (2001)

\bibitem{DBH91}
Davies, M. B., Benz, W.,  Hills, J. G.: ApJ {\bf 381}, 449 (1991)

\bibitem{DBH93}
Davies, M. B., Benz, W.,  Hills, J. G.: ApJ {\bf 411}, 285 (1993)

\bibitem{DBH94}
Davies, M. B., Benz, W.,  Hills, J. G.:  ApJ {\bf 424}, 870 (1994)

\bibitem{DH98}
Davies, M. B. ,  Hansen, B. M. S.: MNRAS {\bf 301}, 15 (1998)

\bibitem{davDPd04}
Davies, M. B., Piotto, G.,  de Angeli, F.: MNRAS {\bf 349}, 129 (2004)

\bibitem{dM06}
de Marchi, F., de Angeli, F., Piotto, G., Carraro, G.,  Davies, M. B.: A\&A {\bf 459}, 489 (2006)

\bibitem{EFT89}
Eggleton, P. P., Fitchett, M. J.,  Tout, C. A.: ApJ {\bf 347}, 998 (1989)

\bibitem{davFPR75}
Fabian, A. C., Pringle, J. E.,  Rees, M. J.:  MNRAS {\bf 172}, 15P (1975)

\bibitem{Ferraro09}
Ferraro, F. R., Beccari, G., Dalessandro, E., et al.:  Nature {\bf 462}, 1028 (2009)

\bibitem{GP08}
Glebbeek, E. ,  Pols, O. R.: A\&A {\bf 488}, 1017 (2008)

\bibitem{GPH08}
Glebbeek, E., Pols, O. R.,  Hurley, J. R.: A\&A {\bf 488}, 1007 (2008)

\bibitem{Heggie75}
Heggie, D. C.: MNRAS {\bf 173}, 729 (1975)

\bibitem{HMG92}
Hut, P., McMillan, S., Goodman, J., et al.: PASP {\bf 104}, 981 (1992)

\bibitem{HMR92}
Hut, P., McMillan, S.,  Romani, R. W.: ApJ {\bf 389}, 527 (1992)

\bibitem{HV83}
Hut, P. ,  Verbunt, F.: Nature {\bf 301}, 587 (1983)

\bibitem{KLS09}
Knigge, C., Leigh, N.,  Sills, A.: Nature {\bf 457}, 288 (2009)

\bibitem{LKS13}
Leigh, N., Knigge, C., Sills, A., et al.: MNRAS {\bf 428}, 897 (2013)

\bibitem{davLeonard89}
Leonard, P. J. T.: AJ {\bf 98}, 217 (1989)

\bibitem{LRS95}
Lombardi, Jr., J. C., Rasio, F. A.,  Shapiro, S. L.: ApJ {\bf 445}, L117 (1995)

\bibitem{LRS96}
Lombardi, Jr., J. C., Rasio, F. A.,  Shapiro, S. L.: ApJ {\bf 468}, 797(1996)

\bibitem{Lom02}
Lombardi, Jr., J. C., Warren, J. S., Rasio, F. A., Sills, A.,  Warren, A. R.: ApJ {\bf 568}, 939 (2002)

\bibitem{MG09}
Mathieu, R. D. ,  Geller, A. M.: Nature {\bf 462}, 1032 (2009)

\bibitem{davMcCrea64}
McCrea, W. H.: MNRAS {\bf 128}, 147 (1964)

\bibitem{Milone12}
Milone, A. P., Piotto, G., Bedin, L. R., et al.: A\&A {\bf 540}, A16 (2012)

\bibitem{PFa09}
Perets, H. B. ,  Fabrycky, D. C.: ApJ {\bf 697}, 1048 (2009)

\bibitem{Piotto04}
Piotto, G., De Angeli, F., King, I. R., et al.: ApJ {\bf 604}, L109 (2004)

\bibitem{PS00}
Preston, G. W. ,  Sneden, C.: AJ {\bf 120}, 1014 (2000)

\bibitem{SanBH97}
Sandquist, E. L., Bolte, M.,  Hernquist, L.: ApJ {\bf 477}, 335 (1997)

\bibitem{SP93}
Sigurdsson, S. ,  Phinney, E. S.: ApJ {\bf 415}, 631(1993)

\bibitem{SAD05}
Sills, A., Adams, T.,  Davies, M. B.: MNRAS {\bf 358}, 716 (2005)

\bibitem{SADB02}
Sills, A., Adams, T., Davies, M. B.,  Bate, M. R.: MNRAS {\bf 332}, 49 (2002)

\bibitem{davSills01}
Sills, A., Faber, J. A., Lombardi, Jr., J. C., Rasio, F. A.,  Warren, A. R.: ApJ {\bf 548}, 323 (2001)

\bibitem{SGCR13}
Sills, A., Glebbeek, E., Chatterjee, S.,  Rasio, F. A.: ApJ {\bf 777}, 105  (2013)

\bibitem{SKL09}
Sills, A., Karakas, A.,  Lattanzio, J.: ApJ {\bf 692}, 1411 (2009)

\bibitem{davSills97}
Sills, A., Lombardi, Jr., J. C., Bailyn, C. D., et al.: ApJ {\bf 487}, 290 (1997)

\bibitem{SPC03}
Sneden, C., Preston, G. W.,  Cowan, J. J.: ApJ {\bf 592}, 504 (2003)

\bibitem{TF05}
Tanikawa, A. ,  Fukushige, T.: PASJ {\bf 57}, 155
(2005)

\bibitem{Vilhu82}
Vilhu, O.: A\&A {\bf 109}, 17 (1982)

\end{thebibliography}

==> refdeng.tex <==
\begin{thebibliography}{99}
\bibitem{AL95} Ahumada, J. \& Lapasset, E.: A\&AS \textbf{109}, 375 (1995)
\bibitem{AL07} Ahumada, J. \& Lapasset, E.: A\&A \textbf{463}, 789 (2007)
\bibitem{BH87} Benz, W. \& Hills, J.G.: ApJ \textbf{323}, 614 (1987)
\bibitem{BH92} Benz, W. \& Hills, J.G.: ApJ \textbf{389}, 546 (1992)
\bibitem{Bertelli+94} Bertelli, G., Bressan, A., Chiosi, C., Fagotto, F., Nasi, E.: A\&AS \textbf{106}, 275 (1994)
\bibitem{BA86} Bica, E., \& Alloin, D.: A\&AS \textbf{66}, 171 (1986)
%\bibitem{science-journal} Bica, E., Geisler, D., Dottori, H., Clari\'a, J.J., Piatti, A.E., Santos~Jr., J.F.C.: Ages and Metallicities of Star Clusters and Surrounding Fields in the Outer Disk of the Large Magellanic Cloud. AJ \textbf{116}, 723--737 (1998)
\bibitem{BC03} Bruzual, G. \& Charlot, S.: MNRAS \textbf{344}, 1000 (2003)
\bibitem{Chabrier03} Chabrier, G.: PASP \textbf{115}, 763 (2003)
\bibitem{CH09} Chen, X. \& Han, Z.: MNRAS \textbf{395}, 1822 (2009)
\bibitem{Dabringhausen+08} Dabringhausen, J., Hilker, M., Kroupa, P.: MNRAS \textbf{386}, 864 (2008)
\bibitem{Deng+99} Deng, L., Chen, R., Liu, X.S., Chen, J.S.: ApJ \textbf{524}, 824 (1999)
\bibitem{Deng+13} Deng, L., Xin, Y. , Zhang, X. B., Li, Y.; Jiang, X.J.; Wang, G.M.; Wang, K.; Zhou, J.L.; Yan, Z.Z.; Luo, Z.Q.: IAUS, \textbf{288}, 318 (2013) 
\bibitem{Fan+96} Fan, X., Burstein, D., Chen, J.S., Zhu, J., Jiang, Z., Wu, H., Yan, H., Zheng, Z., Zhou, X. Fang, L.Z., et al.: AJ \textbf{112}, 628 (1996)
\bibitem{Ferraro+09} Ferraro, F.R., Beccari, G., Dalessandro, E., Lanzoni, B., Sills, A., Rood, R.T., Pecci, F.F., Karakas, A.I., Miocchi, P., Bovinelli, S.: Nature \textbf{462}, 1028 (2009)
\bibitem{Girardi+00} Girardi, L., Bressan, A., Bertelli, G., Chiosi, C.: A\&AS \textbf{141}, 371 (2000)
\bibitem{Kroupa01} Kroupa, P.: MNRAS \textbf{322}, 231 (2001)
\bibitem{Kroupa02} Kroupa, P.: Science \textbf{295}, 82 (2002)
\bibitem{STELIB} Le~Borgne, J.F., Bruzual, G., Pello, R., Lancon, A., Rocca-Volmerange, B., Sanahuja, B., Schaerer, D., Soubiran, C., Vilchez-Gomez, R.: A\&A \textbf{402}, 433 (2003)
\bibitem{Leitherer+99} Leitherer, C., Schaerer, D., Goldader, J.D., Gonz\'alez~Delgado, R.M., Robert, C., Kune, D.F., de~Mello, D.F., Devost, D., Heckman, T.M.: ApJS \textbf{123}, 3 (1999)
\bibitem{Lejeune+97} Lejeune, T., Cuisinier, F., Buser, R.: A\&AS \textbf{125}, 229 (1997)
\bibitem{LL92} Leonard, P.J.T. \& Linnell, A.P.: AJ \textbf{103}, 1928 (1992)
\bibitem{LiHan08} Li, Z. \& Han, Z.: ApJ \textbf{685}, 225 (2008)
\bibitem{Liu+08} Liu, G.Q., Deng, L., Ch\'avez, M., Bertone, E., Davo, A.H., Mata-Ch\'avez, M.D.: MNRAS \textbf{390}, 665 (2008)
\bibitem{MPG06} Mackey, M.C., Payne, M.J., Gilmore, G.F.: MNRAS \textbf{369}, 921 (2006)
\bibitem{Mapelli+09} Mapelli, M., Ripamonti, E., Battaglia, G., Tolstoy, E., Irwin, M.J., Moore, B., Sigurdsson, S.: MNRAS \textbf{396}, 1771 (2009)
\bibitem{MHS86} Mateo, M., Hodeg, P., Schommer, R.A.: ApJ \textbf{311}, 113 (1986)
\bibitem{McCrea64} McCrea, W.H.: MNRAS \textbf{128}, 147 (1964)
%\bibitem{science-journal} Piatti, A.E., Santos~Jr., J.F.C., Clari\'a, J.J., Bica, E., Ahumada, A.V., Parisi, M.C.: Integrated spectral analysis of 18 concentrated star clusters in the Small Magellanic Cloud. A\&A \textbf{440}, 111--120 (2005)
\bibitem{Pickles98} Pickles, A.J.: PASP \textbf{110}, 863 (1998)
\bibitem{Piotto08} Piotto, G.: IAUS \textbf{246}, 141 (2008) 
\bibitem{Piotto+02} Piotto, G., King, I.P., Djorgovski, S.G., Sosin, C., Zoccali, M., Saviane, I., De~Angeli, F., Riello, M., Recio-Blanco, A., Rich, R.M., Meylan, G., Renzini, A.: A\&A \textbf{391}, 945 (2002)
\bibitem{Salpeter55} Salpeter, E.E.: ApJ \textbf{121}, 161 (1955)
\bibitem{SS00} Shetrone, M.D. \& Sandquist, E.L.: AJ \textbf{120}, 1913 (2000)
\bibitem{Stryker93} Stryker, L.L.: PASP \textbf{105}, 1081 (1993)
\bibitem{Thomas+03} Thomas, D., Maraston, C., Bender, R.: MNRAS \textbf{339}, 897 (2003)
\bibitem{Vazdekis99} Vazdekis, A.: ApJ \textbf{513} 224 (1999)
\bibitem{Worthey94} Worthey, G.: ApJS \textbf{95}, 107 (1994)
\bibitem{XD05} Xin, Y. \& Deng, L.: ApJ \textbf{619}, 824 (2005)
\bibitem{Xin+11} Xin, Y., Deng, L., de~Grijs, R., Kroupa, P.: MNRAS \textbf{411}, 761 (2011)
\bibitem{Xin+08} Xin, Y., Deng, L., de~Grijs, R., Mackey, A.D., Han, Z.: MNRAS \textbf{384}, 410 (2008)
\bibitem{Xin+07} Xin, Y., Deng, L., Han, Z.: ApJ \textbf{660}, 319 (2007)
\bibitem{Yi03} Yi, S.K.: ApJ \textbf{582}, 202 (2003) 

\end{thebibliography}


==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%
% sample references
% 
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...´': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}


==> referenc0.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...´': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}


==> referenc1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%

\begin{thebibliography}{99.}%
\bibitem{science-journal} Ahumada, J. \& Lapasset, E.: Catalogue of blue stragglers in open clusters. A\&AS \textbf{109}, 375--382 (1995)
\bibitem{science-journal} Ahumada, J. \& Lapasset, E.: New catalogue of blue stragglers in open clusters. A\&A \textbf{463}, 789--797 (2007)
\bibitem{science-journal} Benz, W. \& Hills, J.G.: Three-dimensional hydrodynamical simulations of stellar collisions. I - Equal-mass main-sequence stars. ApJ \textbf{323}, 614--628 (1987)
\bibitem{science-journal} Benz, W. \& Hills, J.G.: Three--dimensional hydrodynamical simulations of colliding stars . III -- Collisions and tidal captures of unequal--mass main--sequence stars. ApJ \textbf{389}, 546--557 (1992)
\bibitem{science-journal} Bertelli, G., Bressan, A., Chiosi, C., Fagotto, F., Nasi, E.: Theoretical isochrones from models with new radiative opacities. A\&AS \textbf{106}, 275--302 (1994)
\bibitem{science-journal} Bica, E., \& Alloin, D.: A grid of star cluster properties for stellar population synthesis. A\&AS \textbf{66}, 171--179 (1986)
\bibitem{science-journal} Bica, E., Geisler, D., Dottori, H., Clari\'a, J.J., Piatti, A.E., Santos~Jr., J.F.C.: Ages and Metallicities of Star Clusters and Surrounding Fields in the Outer Disk of the Large Magellanic Cloud. AJ \textbf{116}, 723--737 (1998)
\bibitem{science-journal} Bruzual, G. \& Charlot, S.: Stellar population synthesis at the resolution of 2003. MNRAS \textbf{344}, 1000--1028 (2003)
\bibitem{science-journal} Chabrier, G.: Galactic Stellar and Substellar Initial Mass Function. PASP \textbf{115}, 763--795 (2003)
\bibitem{science-journal} Chen, X. \& Han, Z.: Primordial binary evolution and blue stragglers. MNRAS \textbf{395}, 1822--1836 (2009)
\bibitem{science-journal} Dabringhausen, J., Hilker, M., Kroupa, P.: From star clusters to dwarf galaxies: the properties of dynamically hot stellar systems. MNRAS \textbf{386}, 864--886 (2008)
\bibitem{science-journal} Deng, L., Chen, R., Liu, X.S., Chen, J.S.: The Blue Stragglers in M67 and Single-Population Synthesis. ApJ \textbf{524}, 824--830 (1999)
\bibitem{science-journal} Deng, L., Xin, Y. , Zhang, X. B., Li, Y.; Jiang, X.J.; Wang, G.M.; Wang, K.; Zhou, J.L.; Yan, Z.Z.; Luo, Z.Q.: SONG China project - participating in the global network, IAUS, \textbf{288}, 318--319 (2013) 
\bibitem{science-journal} Fan, X., Burstein, D., Chen, J.S., Zhu, J., Jiang, Z., Wu, H., Yan, H., Zheng, Z., Zhou, X. Fang, L.Z., and 16 coauthors: Deep Wide-Field Spectrophotometry of the Open Cluster M67. AJ \textbf{112}, 628--648 (1996)
\bibitem{science-journal} Ferraro, F.R., Beccari, G., Dalessandro, E., Lanzoni, B., Sills, A., Rood, R.T., Pecci, F.F., Karakas, A.I., Miocchi, P., Bovinelli, S.: Two distinct sequences of blue straggler stars in the globular cluster M~30. Natur \textbf{462}, 1028--1031 (2009)
\bibitem{science-journal} Girardi, L., Bressan, A., Bertelli, G., Chiosi, C.: Evolutionary tracks and isochrones for low- and intermediate-mass stars: From 0.15 to 7 Msun, and from Z=0.0004 to 0.03. A\&AS \textbf{141}, 371--383 (2000)
\bibitem{science-journal} Kroupa, P.: On the variation of the initial mass function. MNRAS \textbf{322}, 231--246 (2001)
\bibitem{science-journal} Kroupa, P.: The Initial Mass Function of Stars: Evidence for Uniformity in Variable Systems. Sci \textbf{295}, 82--91 (2002)
\bibitem{science-journal} Le~Borgne, J.F., Bruzual, G., Pello, R., Lancon, A., Rocca--Volmerange, B., Sanahuja, B., Schaerer, D., Soubiran, C., Vilchez--Gomez, R.: STELIB: A library of stellar spectra at R$\sim$2000. A\&A \textbf{402}, 433--442 (2003)
\bibitem{science-journal} Leitherer, C., Schaerer, D., Goldader, J.D., Gonz\'alez~Delgado, R.M., Robert, C., Kune, D.F., de~Mello, D.F., Devost, D., Heckman, T.M.:Starburst99: Synthesis Models for Galaxies with Active Star Formation. ApJS \textbf{123}, 3--40 (1999)
\bibitem{science-journal} Lejeune, T., Cuisinier, F., Buser, R.: Standard stellar library for evolutionary synthesis. I. Calibration of theoretical spectra. A\&AS \textbf{125}, 229--246 (1997)
\bibitem{science-journal} Leonard, P.J.T. \& Linnell, A.P.: On the possibility of a collisional origin for the blue stragglers and contact binaries in the old open clusters M67 and NGC 188. AJ \textbf{103}, 1928--1944 (1992)
\bibitem{science-journal} Liu, G.Q., Deng, L., Ch\'avez, M., Bertone, E., Davo, A.H., Mata--Ch\'avez, M.D.: A spectroscopic study of the blue stragglers in M67. MNRAS \textbf{390}, 665--674 (2008)
\bibitem{science-journal} Mackey, M.C., Payne, M.J., Gilmore, G.F.: Photometry of Magellanic Cloud clusters with the Advanced Camera for Surveys -- II. The unique LMC cluster ESO 121--SC03. MNRAS \textbf{369}, 921--932 (2006)
\bibitem{science-journal} Mapelli, M., Ripamonti, E., Battaglia, G., Tolstoy, E., Irwin, M.J., Moore, B., Sigurdsson, S.: Blue straggler stars in dwarf spheroidal galaxies -- II. Sculptor and Fornax. \textbf{396}, 1771--1782 (2009)
\bibitem{science-journal} Mateo, M., Hodeg, P., Schommer, R.A.: CCD photometry of Large Magellanic Cloud clusters. III -- The unique, remote cluster ESO 121--SC03. ApJ \textbf{311}, 113--134 (1986)
\bibitem{science-journal} McCrea, W.H.: Extended main-sequence of some stellar clusters. MNRAS \textbf{128}, 147--155 (1964)
\bibitem{science-journal} Piatti, A.E., Santos~Jr., J.F.C., Clari\'a, J.J., Bica, E., Ahumada, A.V., Parisi, M.C.: Integrated spectral analysis of 18 concentrated star clusters in the Small Magellanic Cloud. A\&A \textbf{440}, 111--120 (2005)
\bibitem{science-journal} Pickles, A.J.: A Stellar Spectral Flux Library: 1150-25000 \AA. PASP \textbf{110}, 863--878 (1998)
\bibitem{science-journal} Piotto, G.: Observational Evidence of Multiple Stellar Populations in Globular Clusters. IAUS \textbf{246}, 141--150 (2008) 
\bibitem{science-journal} Piotto, G., King, I.P., Djorgovski, S.G., Sosin, C., Zoccali, M., Saviane, I., De~Angeli, F., Riello, M., Recio-Blanco, A., Rich, R.M., Meylan, G., Renzini, A.: HST color-magnitude diagrams of 74 galactic globular clusters in the HST F439W and F555W bands. \textbf{391}, 945--965 (2002)
\bibitem{science-journal} Salpeter, E.E.: The Luminosity Function and Stellar Evolution. ApJ \textbf{121}, 161--167 (1955)
\bibitem{science-journal} Shetrone, M.D. \& Sandquist, E.L.: Spectroscopy of Blue Stragglers and Turnoff Stars in M67 (NGC~2682). AJ \textbf{120}, 1913--1924 (2000)
\bibitem{science-journal} Stryker, L.L.: Blue stragglers. PASP \textbf{105}, 1081--1100 (1993)
\bibitem{science-journal} Thomas, D., Maraston, C., Bender, R.: Stellar population models of Lick indices with variable element abundance ratios. MNRAS \textbf{339}, 897--911 (2003)
\bibitem{science-journal} Vazdekis, A.: Evolutionary Stellar Population Synthesis at 2 $\AA$ Spectral Resolution. ApJ \textbf{513} 224--241 (1999)
\bibitem{science-journal} Worthey, G.: Comprehensive stellar population models and the disentanglement of age and metallicity effects. ApJS \textbf{95}, 107--149 (1994)
\bibitem{science-journal} Xin, Y. \& Deng, L.: Blue Stragglers in Galactic Open Clusters and Integrated Spectral Energy Distributions. ApJ \textbf{619}, 824--838 (2005)
\bibitem{science-journal} Xin, Y., Deng, L., de~Grijs, R., Mackey, A.D., Han, Z.: Simple stellar population models as probed by the Large Magellanic Cloud star cluster ESO 121-SC03. MNRAS \textbf{384}, 410--419 (2008)
\bibitem{science-journal} Xin, Y., Deng, L., Han, Z.: Blue Straggler Stars in Galactic Open Clusters and the Simple Stellar Population Model. ApJ \textbf{660}, 319--329 (2007)
\bibitem{science-journal} Yi, S.K.: Uncertainties of Synthetic Integrated Colors as Age Indicators. ApJ \textbf{582}, 202--214 (2003) 

\end{thebibliography}


==> refferraro.tex <==
\begin{thebibliography}{}

\bibitem{anderson02} Anderson, J.: Omega
  Centauri, A Unique Window into Astrophysics, ASP 265, 87 (2002)

\bibitem{auriere90} Auriere, M., Lauzeral, C.,
  Ortolani, S.: Nature {\bf  344}, 638 (1990)

\bibitem{bai95} Bailyn, C. D.:  A\&ARA {\bf 33}, 133 (1995)

\bibitem{bec06} Beccari, G., Ferraro, F.~R.,
  Lanzoni, B.,  Bellazzini, M.: ApJL {\bf  652}, L121 (2006)

\bibitem{bec07} Beccari. G., et al.: ApJ {\bf 
  679}, 712 (2007)

\bibitem{beccari11pal14} Beccari, G., Sollima,
  A., Ferraro, F.~R., et al.: ApJL {\bf  737}, L3 (2011)

\bibitem{benz87} Benz, W.,  Hills, J. G.: 
  ApJ {\bf  323}, 614 (1987)

\bibitem{bolte93} Bolte, M., Hesser, J.~E., 
 Stetson, P.~B.: ApJL {\bf  408}, L89 (1993)

\bibitem{buon94} Buonanno, R., Corsi, C.E.,
  Buzzoni, A., Cacciari, C., Ferraro, F.R., Fusi Pecci, F.:
  A\&A {\bf  290}, 69 (1994)

\bibitem{cariulo03} Cariulo, P., Degl'Innocenti,
  S.  Castellani, V.: A\&A {\bf  412}, 1121 (2003)

\bibitem{carretta05} Carretta, E., Gratton,
  R. G., Lucatello, S., Bragaglia, A.,  Bonifacio, P.: A\&A {\bf 
  433}, 597 (2005)

\bibitem{contrerasm75} Contreras Ramos,
  R., Ferraro, F.~R., Dalessandro, E., Lanzoni, B.,  Rood,
  R.~T.: ApJ {\bf  748}, 91 (2012)

\bibitem{ema08_6388} Dalessandro, E., et
  al.: A\&A {\bf  677}, 1069 (2008a)

\bibitem{ema_2419} Dalessandro, E., et
  al.: A\&A {\bf  681}, 311 (2008b)
  
 \bibitem{dale2013} Dalessandro, E., 
Ferraro, F.~R., Massari, D., et al.: ApJ {\bf 778}, 135 (2013)


\bibitem{davies04} Davies, M.~B.,
  Piotto, G.,  de Angeli, F.: MNRAS {\bf 349}, 129 (2004)

\bibitem{demarco05} De Marco, O., et
  al.: ApJ {\bf  632}, 894 (2005)

\bibitem{djorgmey93} Djorgovski, S., 
  Meylan, G.: Structure and Dynamics of Globular Clusters, ASP 50,
  325 (1993)

\bibitem{djorgking86} Djorgovski, S., 
  King, I.~R.: ApJL {\bf  305}, L61 (1986)

\bibitem{dotter08} Dotter, A., Sarajedini, A., 
  Yang, S.-C.: AJ {\bf  136}, 1407 (2008)

\bibitem{feparesce93} Ferraro, F. R., 
  Paresce, F.: AJ {\bf  106},154 (1993)

\bibitem{fe93} Ferraro F. R., Pecci F. F.,
Cacciari C., Corsi C., Buonanno R., Fahlman G. G., Richer H. B.: 
AJ {\bf  106}, 2324 (1993)

\bibitem{fe95} Ferraro, F. R., Fusi Pecci, F.,
   Bellazzini, M.: A\&A {\bf  294}, 80 (1995)

\bibitem{fe97} Ferraro, F. R., et
al.: Paltrinieri, B., Fusi Pecci, F., Cacciari, C., Dorman, B., Rood,
R. T., Buonanno, R., Corsi, C. E., Burgarella, D.,  Laget, M.:
A\&A {\bf  324}, 915 (1997; F97)

\bibitem{fe99} Ferraro, F. R., Paltrinieri, B.,
  Rood, R. T.,  Dorman, B.: ApJ {\bf  522}, 983 (1999a)

\bibitem{fe03sixGCs} Ferraro, F. R., Sills,
A., Rood, R. T., Paltrinieri, B.,  Buonanno, R. :  ApJ {\bf  588},
464 (2003)

\bibitem{fe036752} Ferraro, F.~R., 
Possenti, A., Sabbi, E., et al.:  ApJ {\bf  595}, 179 (2003)

\bibitem{fe04} Ferraro, F. R., Beccari, G.,
Rood, R. T., Bellazzini, M., Sills, A.,  Sabbi, E.:  ApJ {\bf  603},
127 (2004)

\bibitem{fe06} Ferraro, F. R., Sollima, A.,
Rood, R. T., Origlia, L., Pancino, E.,  Bellazzini, M.:  ApJ {\bf 
638}, 433 (2006a)

\bibitem{fe06COdep} Ferraro, F. R., et
al.:  A\&A {\bf  647}, L53 (2006b)

\bibitem{fe09m30} Ferraro, F.~R., 
Beccari, G., Dalessandro, E., et al.: Nature {\bf 462}, 1028 (2009; F09)

\bibitem{fe12} Ferraro, F.~R., 
Lanzoni, B., Dalessandro, E., et al.: Nature {\bf 492}, 393 (2012; F12)

\bibitem{fp92} Fusi Pecci, F., Ferraro,
F. R., Corsi, C. E., Cacciari, C.,  Buonanno, R.: ApJ {\bf  104},
1831 (1992)

\bibitem{guha94} Guhathakurta, P., Yanny,
  B., Bahcall, J. N., Schneider, D. P.: ApJ {\bf  108}, 1786
(1994)

\bibitem{gilliland98} Gilliland, R.~L., Bono,
G., Edmonds, P.~D., et al.: ApJ {\bf  507}, 818 (1998)

\bibitem{heggie08m4} Heggie, D.~C., 
  Giersz, M.: MNRAS {\bf 389}, 1858 (2008)

\bibitem{hillsday76} Hills, J. G.,  Day,
  C. A.: ApJL {\bf 17}, 87 (1976)

\bibitem{jordi09} Jordi, K., Grebel, E.~K.,
  Hilker, M., et al.: AJ {\bf  137}, 4586 (2009)

\bibitem{knigge09} Knigge, C., Leigh, N., 
  Sills, A.: Nature {\bf 457}, 288 (2009)

\bibitem{lan07M5} Lanzoni, B., Dalessandro,
E., Ferraro, F. R., Mancini, C., Beccari, G., Rood, R. T., Mapelli,
M.,  Sigurdsson, S. : ApJ {\bf  663}, 267 (2007a)

\bibitem{lan071904} Lanzoni, B., et
  al.: A\&A {\bf  663}, 1040 (2007b)

\bibitem{lan07M55} Lanzoni, B., et al.:
  ApJ {\bf  670}, 1065 (2007c)

\bibitem{lan07imbh} Lanzoni, B., 
Dalessandro, E., Ferraro, F.~R., et al.: ApJL {\bf  668}, L139 (2007)

\bibitem{lan13} Lanzoni, B., Mucciarelli, A.,
  Origlia, L., et al.: ApJ {\bf  769}, 107 (2013)

\bibitem{leigh07} Leigh, N., Sills, A., 
 Knigge, C.: ApJ {\bf  661}, 210 (2007)

\bibitem{leigh11} Leigh, N., Sills, A., 
 Knigge, C.: MNRAS {\bf 415}, 3771 (2011)

\bibitem{leigh13} Leigh, N., Knigge, C., 
Sills, A., et al.: MNRAS {\bf 428}, 897 (2013)

\bibitem{leoliv95} Leonard, P. J. T.,  Livio,
  M.:  ApJL {\bf  447}, 121 (1995)

\bibitem{lomb95} Lombardi, J. C. Jr., Rasio,
  F. A.,  Shapiro, S. L.: ApJL {\bf  445}, 117 (1995)

\bibitem{lovisi10} Lovisi, L., Mucciarelli, 
A., Ferraro, F.~R., et al.: ApJL {\bf  719}, 121 (2010)

\bibitem{lovisi12} Lovisi, L., Mucciarelli, A.,
  Lanzoni, B., et al.: ApJ {\bf  754}, 91 (2012)

\bibitem{luc03}Lucatello, S., Gratton,
  R.G.: A\&A {\bf  406}, L691 (2003)

\bibitem{mapelli04} Mapelli, M., Sigurdsson,
S., Colpi, M., Ferraro, F. R., Possenti, A., Rood, R. T., Sills,
A.,  Beccari, G.:  ApJL {\bf  605}, 29 (2004)

\bibitem{mapelli06} Mapelli, M., Sigurdsson,
S., Ferraro, F. R., Colpi, M., Possenti, A.,  Lanzoni, B.:
MNRAS {\bf 373}, 361 (2006)

\bibitem{mapelli09} Mapelli, M., Ripamonti, E.,
  Battaglia, G., et al.: MNRAS {\bf 396}, 1771 (2009)

\bibitem{marinfranch09}
  Mar{\'{\i}}n-Franch, A., Aparicio, A., Piotto, G., et al.:
  ApJ {\bf  694}, 1498 (2009)

\bibitem{mathieu09} Mathieu, R.~D., 
  Geller, A.~M.: Nature {\bf 462}, 1032 (2009)

\bibitem{mcrea64} McCrea, W. H.: MNRAS {\bf 128}, 147 (1964)

\bibitem{mlvdm05} McLaughlin,
  D.~E.,  van der Marel, R.~P.: A\&A {\bf 161}, 304 (2005)

\bibitem{meylanheggie97} Meylan, G., 
  Heggie, D.~C.: A\&A Rev. {\bf 8}, 1 (1997)

\bibitem{milone12} Milone, A.~P., Piotto, G.,
  Bedin, L.~R., et al.: A\&A {\bf  540}, A16 (2012)

\bibitem{monelli12} Monelli, M., Cassisi, S.,
  Mapelli, M., et al.: ApJ {\bf  744}, 157 (2012)

\bibitem{moretti08} Moretti, A., de Angeli, F.,
   Piotto, G.: A\&A {\bf  483}, 183 (2008)

\bibitem{paresce91}Paresce, F., Meylan, G.,
  Shara, M., et al.:  Nature {\bf  352}, 297 (1991)

\bibitem{pietrinferni06} Pietrinferni, A.,
  Cassisi, S., Salaris, M.,  Castelli, F.: ApJ {\bf  642}, 797 (2006)

\bibitem{piotto04} Piotto, G., et al.: 
  ApJ {\bf  604}, L109 (2004)

\bibitem{quievy09} Quievy, D., Charbonneau, P.,
  Michaud, G.,  Richer, J.: A\&A {\bf  500}, 1163 (2009)

\bibitem{renzfusi88} Renzini, A.,  Fusi
  Pecci, F.: A\&ARA {\bf 26}, 199 (1988)

\bibitem{sabbi04} Sabbi, E., Ferraro, F. R., Sills, A.,
 Rood, R. T.: ApJ {\bf  617}, 1296 (2004)

\bibitem{sand53} Sandage A. R.: AJ {\bf  58}, 61 (1953)

\bibitem{saraj93} Sarajedini, A.: Blue
  Stragglers, ASP {\bf 53}, 14 (1993)

\bibitem{saraj07} Sarajedini, A., Bedin,
  L.~R., Chaboyer, B., et al.: AJ {\bf  133}, 1658 (2007)

\bibitem{sarna96} Sarna, M. J.,  de Greve,
  J. P.: QJRAS {\bf 37}, 11 (1996)

\bibitem{shara97} Shara, M. M., Saffer, R. A., 
  Livio, M.: ApJ {\bf  489}, L59 (1997)

\bibitem{sigurd94}Sigurdsson, S., Davies,
  M.B.,  Bolte, M.: ApJL {\bf  431}, 115 (1994)

\bibitem{sills05} Sills, A., Adams, T.,  Davies,
  M.~B.: MNRAS {\bf 358}, 716 (2005)

\bibitem{sills09} Sills, A., Karakas, A., 
  Lattanzio, J.: ApJ {\bf  692}, 1411 (2009)

\bibitem{sollima08} Sollima, A. et al.:
  A\&A {\bf  481}, 701 (2008)

\bibitem{tian06} Tian, B., Deng, L., Han, Z., 
  Zhang, X.~B.: A\&A {\bf  455}, 247 (2006)

\bibitem{w06} Warren, S. R., Sandquist, E. L.,
   Bolte, M.: ApJ {\bf  648}, 1026 (2006)

\bibitem{zaggia97} Zaggia, S. R., Piotto, G. 
  Capaccioli M.: A\&A {\bf  327}, 1004 (1997)

\bibitem{zinnsearle76} Zinn, R.,  Searle, L.: 
  ApJ {\bf  209}, 734 (1976)

\end{thebibliography} 



==> refivanova.tex <==
\begin{thebibliography}{99}
\providecommand{\url}[1]{{#1}}
\providecommand{\urlprefix}{URL }
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{DOI \discretionary{}{}{}#1}\else
  \providecommand{\doi}{DOI \discretionary{}{}{}\begingroup
  \urlstyle{rm}\Url}\fi


\bibitem{Beg79}
 {Begelman}, M. C.: \mnras \textbf{187}, 237 (1979)

\bibitem{2008ApJS..174..223B}
Belczynski, K.,  {Kalogera}, V.,  {Rasio}, F.~A. et al.:
%R.~E.  {Taam}, A.  	{Zezas}, T.  {Bulik}, T.~J.  {Maccarone}, N.{Ivanova}
 \apjs \textbf{174}, 223 (2008)
%      \doi = {10.1086/521026}

\bibitem{Dalsgaard2011} 
Christensen-Dalsgaard, J.: in Progress in Solar/Stellar Physics with 
Helio- and Asteroseismology, ASP Conf. \textbf{462}, 503 (2012)

\bibitem{dar79}
{Darwin}, G. H.: Proc. Roy. Soc. London \textbf{29}, 168 (1879)

\bibitem{2003ApJ...598.1217D}
{Deloye}, C. J.,~{Bildsten}, L.: \apj \textbf{598}, 1217 (2003)
%\newblock \doi{10.1086/379063}

\bibitem{dem91}
{Demircan}, O., {Kahraman}, G.: \apss \textbf{181}, 313 (1991)
%\newblock \doi{10.1007/BF00639097}

\bibitem{1971MNRAS.151..351E}
 {Eggleton}, P. P.: \mnras \textbf{151}, 351 (1971)

\bibitem{1972MNRAS.156..361E}
{Eggleton}, P. P.: \mnras \textbf{156}, 361 (1972)

\bibitem{1973MNRAS.163..279E}
{Eggleton}, P. P.: \mnras \textbf{163}, 279 (1973)

\bibitem{Eggl83}
{Eggleton}, P. P.: \apj \textbf{268}, 368 (1983)
%\newblock \doi{10.1086/160960}

\bibitem{2000NewAR..44..111E}
{Eggleton}, P. P.: New Astronomy Reviews \textbf{44}, 111 (2000)
%\newblock \doi{10.1016/S1387-6473(00)00023-3}

\bibitem{Eggl06}
{Eggleton}, P. P.: Evolutionary Processes in Binary and Multiple Stars, Cambridge University Press
  (2006)

\bibitem{2012JASS...29..145E}
{Eggleton}, P. P.: Journal of Astronomy and Space Sciences \textbf{29}, 145
  (2012)
%\newblock \doi{10.5140/JASS.2012.29.2.145}

\bibitem{1973AA....23..325E}
{Eggleton}, P. P., {Faulkner}, J.,~{Flannery}, B. P.: \aap \textbf{23}, 325 (1973)

\bibitem{2006Ap&SS.304...75E}
{Eggleton}, P. P., {Kisseleva-Eggleton}, L.: \apss \textbf{304}, 75 (2006)
%\newblock \doi{10.1007/s10509-006-9078-z}

\bibitem{2011ascl.soft07008E}
{Eggleton}, P. P., {Tout}, C., {Pols}, O. R., et al.:
%R.~{Izzard}, J.~{Eldridge}, P.~{Lesaffre}, R.~{Stancliffe}, R.~{Church}, H.~{Lau}:
{STARS: A Stellar Evolution Code}, Astrophysics Source Code Library (2011)

\bibitem{2007ApJ...669.1298F}
{Fabrycky}, D., {Tremaine}, S.: \apj \textbf{669}, 1298 (2007)
%\newblock \doi{10.1086/521702}

\bibitem{Ge2010}
H.~{Ge}, M. S. {Hjellming}, R. F. {Webbink}, X.~{Chen}, Z.~{Han}: \apj
  \textbf{717}, 724 (2010)
%\newblock \doi{10.1088/0004-637X/717/2/724}

\bibitem{2013EPJWC..4304001G}
 Geier, S.: European Physical Journal Web of Conferences \textbf{43}, 4001 (2013)
%\doi = {10.1051/epjconf/20134304001}
      
\bibitem{2008AA...488.1007G}
~{Glebbeek}, E.,  {Pols}, O. R., {Hurley}, J. R.: \aap \textbf{488}, 1007 (2008)
%\newblock \doi{10.1051/0004-6361:200809930}

\bibitem{heinke2013}
 {Heinke}, C. O., {Ivanova}, N.,  {Engel}, M. C., et al.:
%K.~{Pavlovskii}, G.R. {Sivakoff}, T.F. {Cartwright}, J.C. {Gladstone}: 
  \apj \textbf{768}, 184 (2013)
%\newblock \doi{10.1088/0004-637X/768/2/184}

\bibitem{Hje87}
 {Hjellming}, M. S., {Webbink}, R. F.: \apj \textbf{318}, 794 (1987)
%\newblock \doi{10.1086/165412}

\bibitem{1991ApJ...370..709H}
 {Hjellming}, M. S., {Taam}, R. E.: \apj \textbf{370}, 709 (1991)
%\newblock \doi{10.1086/169854}

\bibitem{iva2002MNRAS.329..897H}
 Hurley, J.~R., {Tout}, C.~A.,  {Pols}, O.~R.: \mnras \textbf{329}, 897 (2002)
%\doi{10.1046/j.1365-8711.2002.05038.x}
      
\bibitem{Hut80}
{Hut}, P.: \aap \textbf{92}, 167 (1980)

\bibitem{2007AA...465..953I}
 {in't Zand}, J. J. M., {Jonker}, P. G. ,  {Markwardt}, C.B.: \aap \textbf{465}, 953
  (2007)
%\newblock \doi{10.1051/0004-6361:20066678}

\bibitem{1997AJ....113.1915I}
 {Innanen}, K. A., {Zheng}, J. Q., {Mikkola}, S.,  {Valtonen}, M.~J.: \aj \textbf{113},
  1915 (1997)
%\newblock \doi{10.1086/118405}

\bibitem{Iva03}
{Ivanova}, N.: DPhil Thesis  (2003)

\bibitem{2008msah.conf..101I}
{Ivanova}, N.: in Multiple Stars Across the H-R Diagram, ESO Symp., Springer-Verlag, p. 101 (2008)
%\newblock \doi{10.1007/978-3-540-74745-1_14}

\bibitem{ips02}
{Ivanova}, N., {Podsiadlowski}, P., {Spruit}, H.: \mnras \textbf{334}, 819 (2002)
%\newblock \doi{10.1046/j.1365-8711.2002.05543.x}

\bibitem{Iva04}
{Ivanova}, N.,  {Taam}, R.E.: \apj \textbf{601}, 1058 (2004)
%\newblock \doi{10.1086/380561}

\bibitem{iva_ce}
{Ivanova}, N., {Justham}, S., {Chen}, X., et al.:
%O.~{De Marco}, C.L. {Fryer},E.~{Gaburov}, H.~{Ge}, E.~{Glebbeek}, Z.~{Han}, X.D. {Li}, G.~{Lu}, T.~{Marsh}, P.~{Podsiadlowski}, A.~{Potter}, N.~{Soker}, R.~{Taam}, T.M. {Tauris}, E.P.J. {van den Heuvel}, R.F. {Webbink}: 
\aapr \textbf{21}, 59  (2013)

\bibitem{kipwei67}
{Kippenhahn}, R., {Weigert}, A.: \zap \textbf{65}, 251 (1967)

\bibitem{Kip67}
{Kippenhahn}, R., {Weigert}, A., {Hofmeister}, E.: Mth. Comp. Phys. \textbf{7},
  129 (1967)

\bibitem{1962AJ.....67..591K}
{Kozai}, Y.: \aj \textbf{67}, 591 (1962)
%\newblock \doi{10.1086/108790}

\bibitem{2008IAUS..250..167L}
  {Langer}, N., {Cantiello}, M.,  {Yoon},  S.-C., et al.: 
%  I. {Hunter}, I. {Brott}, D. {Lennon}, S. {de Mink}, M. {Verheijdt}: 
	in IAU Symposium 250, pp-167 (2008)

\bibitem{ivalau70}
{Lauterborn}, D.: \aap \textbf{7}, 150 (1970)

\bibitem{2002ApJ...568..939L}
 {Lombardi}, Jr., J. C., {Warren},  J.S., {Rasio}, F. A. , {Sills},  A.,  {Warren}, A.~R.:
  \apj \textbf{568}, 939 (2002)
%\newblock \doi{10.1086/339060}

\bibitem{2011ApJ...737...49L}
{Lombardi}, Jr., J. C. , {Holtzman}, W., {Dooley}, K. L. ,~{Gearity},  K., {Kalogera}, V., {Rasio}, F. A.: \apj \textbf{737}, 49 (2011)
%\newblock \doi{10.1088/0004-637X/737/2/49}

\bibitem{1976ApJ...207L..53L}
 {Lubow}, S. H.,  {Shu}, F. H.: \apjl \textbf{207}, L53 (1976)
%\newblock \doi{10.1086/182177}

\bibitem{2011MNRAS.418.1156M}
{Maxted}, P. F. L.,  {Anderson}, D. .,  {Burleigh}, M. R., et al.: 
%A.~{Collier Cameron},U.~{Heber}, B.T. {G{\"a}nsicke}, S.~{Geier}, T.~{Kupfer}, T.R. {Marsh}, G.~{Nelemans}, S.J. {O'Toole}, R.H. {{\O}stensen}, B.~{Smalley}, R.G. {West}:
  \mnras \textbf{418}, 1156 (2011)
%\newblock \doi{10.1111/j.1365-2966.2011.19567.x}

\bibitem{2001ApJ...552..664N}
 {Nelson}, C. A.,  {Eggleton}, P. P.: \apj \textbf{552}, 664 (2001)
%\newblock \doi{10.1086/320560}

\bibitem{Nom79}
{Nomoto}, K., {Nariai}, K., {Sugimoto}, D.: \pasj \textbf{31}, 287 (1979)

\bibitem{1981A&A...102...17P}
Packet, W.: \aap \textbf{102}, 17 (1981)

\bibitem{2012ApJ...760...90P}
 {Passy}, J. C., {Herwig}, F., {Paxton}, B.: \apj \textbf{760}, 90 (2012)
%\newblock \doi{10.1088/0004-637X/760/1/90}

\bibitem{2012ApJ...744...52P}
 {Passy}, J.C., {De Marco}, O.,  {Fryer}, C.L., et al.:
 %F.~{Herwig}, S.~{Diehl}, J.S. {Oishi}, M.M. {Mac Low}, G.L. {Bryan}, G.~{Rockefeller}:
   \apj \textbf{744},
  52 (2012)
%\newblock \doi{10.1088/0004-637X/744/1/52}

\bibitem{pavl_casca}
{Pavlovskii}, K., {Ivanova}, N.:  CASCA meeting (2013)

\bibitem{2013IAUS..291..468P}
{Pavlovskii}, K., {Ivanova}, N.: in IAU Symposium 291, 468 (2013)
%\newblock \doi{10.1017/S1743921312024544}

\bibitem{2013IAUS..290..293P}
{Pavlovskii}, K., {Ivanova}, N.: in IAU Symposium, 290, 293 (2013)
%\newblock \doi{10.1017/S1743921312020078}

\bibitem{MESA1}
{Paxton}, B.,~{Bildsten},  L., {Dotter}, A., et al.:
%F.~{Herwig}, P.~{Lesaffre},F.~{Timmes}: 
  \apjs \textbf{192}, 3 (2011)
%\newblock \doi{10.1088/0067-0049/192/1/3}

\bibitem{MESA2}
Paxton, B., Cantiello, 
M., Arras, P., et al.: \apjs \textbf{208}, 4  (2013)

\bibitem{podsi02}
{Podsiadlowski}, P., {Rappaport}, S.,  {Pfahl}, E. D.: \apj \textbf{565}, 1107
  (2002)
%\newblock \doi{10.1086/324686}

\bibitem{1995MNRAS.274..964P}
 {Pols}, O. R., {Tout}, C. A. ,  {Eggleton}, P. P., {Han}, Z.: \mnras \textbf{274}, 964
  (1995)

\bibitem{2012MNRAS.427.1702R}
{Raymer}, E.: \mnras \textbf{427}, 1702 (2012)
%\newblock \doi{10.1111/j.1365-2966.2012.22090.x}

\bibitem{2012ApJ...746...74R}
 {Ricker}, P. M., {Taam}, R. E.: \apj \textbf{746}, 74 (2012)
%\newblock \doi{10.1088/0004-637X/746/1/74}

\bibitem{1980ApJ...239..937S}
 Shu, F.~H.,   {Lubow}, S.~H., {Anderson}, L.: 
{\apj}, \textbf{239}, 937 (1980)
%\doi = {10.1086/158181}
      
\bibitem{Sob97}
 {Soberman}, G. E., {Phinney}, , E. S.,  {van den Heuvel}, E. P. J.: \aap \textbf{327},
  620 (1997)

\bibitem{2008MNRAS.389.1828S}
 Stancliffe, R.~J.,  Glebbeek, E.:
\mnras \textbf{389}, 1828 (2008)
%\doi = {10.1111/j.1365-2966.2008.13700.x}
      
\bibitem{Tout97}
{Tout}, C.~A.,  {Aarseth}, S.~J.,  {Pols}, O. R., {Eggleton}, P. P.: \mnras \textbf{291},
  732 (1997)
  
\bibitem{2008AA...487.1129V}
{van Rensbergen}, W.,  {De Greve}, J.P., {De Loore}, C., {Mennekens}, N.: \aap
  \textbf{487}, 1129 (2008)
%\newblock \doi{10.1051/0004-6361:200809943}

\bibitem{2011AA...528A..16V}
{van Rensbergen},  W., {De Greve},J.P., ~{Mennekens},  N.,
	{Jansen}, K. , de Loore, C.: 
 {\aap},\textbf{528}, A16 (2011)
%\doi = {10.1051/0004-6361/201015596}
      
\bibitem{webbink1985}
{Webbink}, R.F.: in Stellar evolution and binaries, Cambridge University Press, p.~39 (1985)

\bibitem{woodsmt11}
{Woods}, T.E.,  {Ivanova}, N.: \apjl \textbf{739}, L48 (2011)
%\newblock \doi{10.1088/2041-8205/739/2/L48}

\bibitem{woods11}
{Woods}, T.E., {Ivanova}, N.~, {van der Sluys}, M.V. , {Chaichenets}, S.~: \apj
  \textbf{744}, 12 (2012)
%\newblock \doi{10.1088/0004-637X/744/1/12}

\bibitem{1997MNRAS.292..321Y} Yukawa, H.,  Boffin, H.~M.~J., Matsuda, T. : \mnras \textbf{292}, 321 (1997)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{thebibliography}


==> refknigge.tex <==

\begin{thebibliography}{99.}%
\bibitem{Chat13}Chatterjee, S., Rasio, F.~A., Sills, A., Glebbeek, E.: ApJ  {\bf 777}, 106 (2013)
\bibitem{Clark75}Clark, G.~W.: ApJL {\bf 199}, L143 (1975)
\bibitem{DPd04}Davies, M.~B., Piotto, G.,  de Angeli, F.: MNRAS {\bf 349}, 129 (2004)
\bibitem{Egg89}Eggleton, P.~P., Fitchett, M.~J.,  Tout, C.~A.: ApJ {\bf 347}, 998 (1989)
\bibitem{Egg90}Eggleton, P.~P., Fitchett, M.~J.,  Tout, C.~A.: ApJ {\bf  354}, 387 (1990)
\bibitem{FPR75}Fabian, A.~C., Pringle, J.~E.,  Rees, M.~J.: MNRAS {\bf 172}, 15P (1975)
\bibitem{Fe09}Ferraro, F.~R., Beccari, G., Dalessandro, E., et al.: Nature {\bf 462}, 1028 (2009)
%\bibitem{dummy7}Ferraro, F.~R., Beccari, G., Rood, R.~T., et al.: 2004, ApJ {\bf  603, 127 
\bibitem{Fer97}Ferraro, F.~R., Paltrinieri, B., Fusi Pecci, F., et al.: A\&A {\bf 324}, 915 (1997)
\bibitem{Fer06}Ferraro, F.~R., Sabbi, E., Gratton, R., et al.: ApJL {\bf  647}, L53 (2006)
\bibitem{HPT00}Hurley, J.~R., Pols, O.~R.,  Tout, C.~A.:  MNRAS {\bf  315}, 543 (2000)
\bibitem{Hut92}Hut, P., McMillan, S.,  Goodman, J., et al.: PASP {\bf  104}, 981 (1992)
\bibitem{Katz75}Katz, J.~I.: Nature {\bf  253}, 698 (1975)
\bibitem{Kni09}Knigge C., Leigh N., Sills A.: Nature {\bf  457}, 288 (2009) 
\bibitem{Lan07a}Lanzoni, B., Dalessandro, E., Ferraro, F.~R., et al.: ApJ {\bf  663}, 267 (2007a)
\bibitem{Lan07b}Lanzoni, B., Dalessandro, E., Perina, S., et al.: ApJ {\bf  670}, 1065 (2007b)
\bibitem{LG12}Leigh N., Geller A.~M.: MNRAS {\bf  425}, 2369 (2012)
\bibitem{Leigh13}Leigh N., Knigge C., Sills A., et al.: MNRAS {\bf  428}, 897 (2013)
\bibitem{LSK07}Leigh N., Sills A., Knigge C.: ApJ {\bf  661}, 210 (2007)
\bibitem{LSK08}Leigh N., Sills A., Knigge C.: ApJ {\bf  678}, 564 (2008)
\bibitem{LSK11}Leigh N., Sills A., Knigge C.: MNRAS {\bf 415}, 3771 (2011)
\bibitem{LS11}Leigh N., Sills A.: MNRAS {\bf 410}, 2370 (2011)
\bibitem{Mason10}Mason, E., Diaz, M., Williams, R.~E., Preston, G.,  Bensby, T.:  A\&A {\bf 516}, A108 (2010)
\bibitem{Ma04}Mapelli, M., Sigurdsson, S., Colpi, M., et al.: ApJL {\bf 605}, L29 (2004)
\bibitem{Ma06}Mapelli, M., Sigurdsson, S., Ferraro, F.~R., et al.: MNRAS {\bf 373}, 361 (2006)
\bibitem{Mil12}Milone, A.~P., Piotto, G., Bedin, L.~R., et al.: A\&A {\bf 540}, A16 (2012)
\bibitem{Mil08}Milone, A.~P., Piotto, G., Bedin, L.~R.,  Sarajedini, A.: Mem. Soc. Astron. Ital. {\bf 79}, 623 (2008)
\bibitem{Nakano2008}Nakano, S., Nishiyama, K., Kabashima, F., et al.: IAU Circ. {\bf 8972}, 1 (2008)
\bibitem{Pio04}Piotto, G., De Angeli, F., King, I.~R., et al.: ApJL {\bf 604}, L109 (2004)
\bibitem{Pio02}Piotto, G., King, I.~R., Djorgovski, S.~G., et al.: A\&A {\bf 391}, 945 (2002)
\bibitem{PH06}Pooley, D.,  Hut, P.: ApJL {\bf 646}, L143 (2006)
\bibitem{Po03}Pooley, D., Lewin, W.~H.~G., Anderson, S.~F., et al.: ApJL {\bf 591}, L131 (2003)
\bibitem{SFS04}Sabbi, E., Ferraro, F.~R., Sills, A.,  Rood, R.~T.: ApJ {\bf 617}, 1296 (2004)
\bibitem{SBC07}Sarajedini, A., Bedin, L.~R., Chaboyer, B., et al.: AJ {\bf 133}, 1658 (2007)
\bibitem{Si01}Sills, A., Faber, J.~A., Lombardi, J.~C., Jr., Rasio, F.~A.,  Warren, A.~R.: ApJ {\bf 548}, 323 (2001)
\bibitem{Si13}Sills, A., Glebbeek, E., Chatterjee, S.,  Rasio, F.~A.: ApJ {\bf 777}, 105 (2013)
\bibitem{SBFF07}Sollima, A., Beccari, G., Ferraro, F.~R., Fusi Pecci, F.,  Sarajedini, A.: MNRAS {\bf  380}, 781 (2007)
\bibitem{SBFF08}Sollima, A., Lanzoni, B., Beccari, G., Ferraro, F.~R.,  Fusi Pecci, F.: A\&A {\bf 481}, 701 (2008)
\bibitem{Ty11}Tylenda, R., Hajduk, M., Kami{\'n}ski, T., et al.: A\&A {\bf 528}, A114 (2011)
\bibitem{Udalski2003}Udalski, A.: Acta Astronomica {\bf 53}, 291 (2003)
\bibitem{WSB06}Warren, S.~R., Sandquist, E.~L.,  Bolte, M.: ApJ {\bf 648}, 1026 (2006)
\end{thebibliography}

==> refmathieu.tex <==
\begin{thebibliography}{99}
\bibitem{AL1995}  Ahumada, J.,  Lapasset, E.: A\&AS {\bf 109}, 375 (1995)
\bibitem{AL2007} Ahumada, J.,  Lapasset, E.:  A\&A {\bf 463}, 789 (2007)
\bibitem{Aarseth2003}  Aarseth, S.~J.:
Gravitational N-Body Simulations, Cambridge University Press (2003)
\bibitem{Belczynsky2008} Belczynski, K., Kalogera, V.,  Rasio, F.,  Taam, R. E.,  Zezas, A.,  Bulik, T., Maccarone, T. J.,  Ivanova, N.: ApJS {\bf 174}, 223 (2008)
\bibitem{BLR2001}  Bergeron, P.,  Leggett, S. K.,  Ruiz, M. T.: ApJS {\bf 133}, 413 (2001)
\bibitem{Bonacic2008} Bona\v ci\'c Marinovi\'c, A. A.,  Glebbeek, E., Pols, O. R.: A\&A {\bf 480}, 797 (2008)
\bibitem{Carneyetal2005}  Carney, B. W., Latham, D. W., Laird,  J. B.: AJ {\bf 129}, 466 (2005)
\bibitem{Carneyetal2001}  Carney, B. W.,  Latham, D. W.,  Laird, J. B., Grant, C. E.,  Morse, J. A.: AJ {\bf
122}, 3419 (2001)
\bibitem{ChenHan2008a}  Chen, X.,  Han, Z.: MNRAS {\bf 384}, 1263 (2008a)
\bibitem{ChenHan2008b} Chen, X.,  Han, Z.: MNRAS {\bf 387}, 1416 (2008b)
\bibitem{Eggleton2011}  Eggleton, P. P.: Evolutionary Processes in Binary and Multiple Stars, Cambridge University Press (2011)
\bibitem{GellerHurleyMathieu2013} Geller, A. M.,  Hurley, J. R.,  Mathieu, R. D.: AJ {\bf 145}, 8 (2013)
\bibitem{GellerMathieu2012}  Geller, A. M., Mathieu, R. D.: AJ {\bf 144}, 54 (2012)
\bibitem{GellerMathieu2011} Geller, A. M., Mathieu, R. D.:  Nature {\bf 478}, 356 (2011)
\bibitem{Geller2010} Geller, A. M., Mathieu, R. D.,  Braden, E. K., et al.: AJ {\bf 139}, 1383 (2010)
\bibitem{Gelleretal2008} Geller, A. M., Mathieu, R. D.,  Harris, H. C., McClure, R. D.: AJ {\bf 135}, 2264 (2008)
\bibitem{Glebbeeketal2008}  Glebbeek, E., Pols, O. R., Hurley, J. R.:  A\&A {\bf 488}, 1007 (2008)
\bibitem{Gondoin2005} Gondoin, P.: A\&A {\bf 438}, 291 (2005)
\bibitem{Goranskij1992}  Goranskij, V. P.,  Kusakin, A. V.,  Mironov, A. V.,  Moshkaljov, V. G., Pas-tukhova, E. N.: Astr. Astroph. Trans. {\bf  2}, 201 (1992)
\bibitem{Gosnelletal2013}  Gosnell, N. M.,  Mathieu, R. D., Geller, A. M., , et al.: ApJL {\bf 783}, 8 (2014)
\bibitem{HillsDay1976}  Hills, J. G., Day, C. A.: ApJL {\bf  17}, 87 (1976)
\bibitem{HjellmingWebbink1987}  Hjellming, M. S., Webbink,  R. F.: ApJ {\bf 318}, 794 (1987)
\bibitem{Hurley2000}  Hurley, J. R.,  Pols, O. R.,  Tout, C. A.: MNRAS {\bf 315}, 543 (2000) 
\bibitem{Hurley2002} Hurley, J. R., Tout, C. A., Pols, O. R.: MNRAS {\bf 329}, 897 (2002)
\bibitem{Hurley2005} Hurley, J. R., Pols, O. R., Aarseth, S.J., Tout, C. A.: MNRAS {\bf 363}, 293 (2005)
\bibitem{Hut2003} Hut, P.: in  Astrophysical Supercomputing using Particle Simulations, IAU Symposium 208, p. 331 (2003) 
\bibitem{JSandage1955}  Johnson, H. L., Sandage, A. R.: ApJ {\bf 121}, 616 (1955)
\bibitem{KippenhahnWeigert1967}  Kippenhahn, R.,  Weigert, A.: Zeit Astrophys. {\bf 65}, 251 (1967)
\bibitem{Kroupa1995}  Kroupa, P.: MNRAS {\bf 277}, 1507 (1995)
\bibitem{LajoieSills2011} Lajoie, C.-P., Sills, A.: ApJ {\bf 726}, 67 (2011)
\bibitem{Latham2007}  Latham, D. W.: Highlights Astron. {\bf 14}, 444 (2007)
\bibitem{Landsman1998}  Landsman, W.,  Bohlin, R. C.,  Neff, S. G., O'Connell, R. W. , Roberts, M. S. , Smith, A. M.,  Stecher, T. P.: AJ {\bf 116}, 789 (1998)
\bibitem{LeighSills2011} Leigh, N. ,  Sills, A.: MNRAS {\bf 410}, 2370 (2011)
\bibitem{LeonardLinnell1992}  Leonard, P. J. T.,  Linnell, A. P.: AJ {\bf 103}, 1928 (1992)
\bibitem{Mardling2001} Mardling, R. A.,  Aarseth, S. J.: MNRAS {\bf 321}, 398 (2001)
\bibitem{Marigoetal2008}  Marigo, P.,  Girardi, L.,  Bressan, A., et al.: A\&A {\bf 482}, 883 (2008)
\bibitem{Mathieu2000} Mathieu, R. D.: in Stellar Clusters and Associations: Convection, Rotation, and Dynamos, ASPC 198, p. 517 (2000)
\bibitem{MathieuGeller2009} Mathieu, R. D., Geller, A. M., Nature {\bf 462}, 1032 (2009)
\bibitem{MathieuLatham1986} Mathieu, R. D., Latham, D. W.: AJ {\bf 92}, 1364 (1986)
\bibitem{Mathys1991} Mathys, G.: A\&A {\bf 245}, 467 (1991)
\bibitem{MazehGoldberg1992} Mazeh, T., Goldberg, D.: ApJ {\bf 394}, 592 (1992)
\bibitem{McCrea1964} McCrea, M. W.: MNRAS {\bf 128}, 147 (1964)
\bibitem{McMillanetal2012} McMillan, S., Portegies Zwart, S., van Elteren, A., Whitehead, A.: in Advances in Computational Astrophysics: Methods, Tools, and Outcome, ASPC 453, p. 129 (2012)
\bibitem{MeibomMathieu2005} Meibom, S.,  Mathieu, R. D.: ApJ {\bf 620}, 970 (2005)
\bibitem{MiloneLatham1992}  Milone, A. A. E.,  Latham, D. W.: in  Evolutionary Processes in Interacting Binary Stars, IAU Symp. 151, p. 475 (1992)
\bibitem{NelsonEggleton2001}  Nelson, C. A.,  Eggleton,  P. P.: ApJ {\bf 552}, 664 (2001)
\bibitem{Paczynski1971} Paczy\'nski, B.: ARA\&A {\bf 9}, 183 (1971)
\bibitem{Passyetal2012}  Passy, J.-C., Herwig, F.,  Paxton, B.: ApJ {\bf 760}, 90 (2012)
\bibitem{Paxtonetal2011}  Paxton, B.,  Bildsten, L.,  Dotter, A.,  Herwig, F.,  Lesaffre, P.,  Timmes, F.: ApJS {\bf 192}, 3 (2011)
\bibitem{PeretsFabrycky2009}  Perets,  H. B.,  Fabrycky,  D. C.: ApJ {\bf 697}, 1048 (2009)
\bibitem{PeretsKratter2012}  Perets, H. B.,  Kratter, K. M.: ApJ {\bf 760}, 99 (2012)
\bibitem{Plataisetal2003} Platais, I.,   Kozhurina-Platais, V.,  Mathieu, R. D.,  Girard, T. M.,  van Altena, W. F.: AJ {\bf 126}, 2922 (2003)
\bibitem{Raghavan2010}  Raghavan, D.,  McAlister, H. A.,  Henry, T. J., et al.: ApJS {\bf 190}, 1 (2010)
\bibitem{Sandage1953}  Sandage, A. R.: AJ {\bf 58}, 61 (1953)
\bibitem{Sandquistetal2003}  Sandquist, E. L.,  Latham, D. W.,  Shetrone, M. D.,  Milone, A. A. E.: AJ {\bf 125}, 810 (2003)
\bibitem{Sarajedinietal1999}  Sarajedini, A., von Hippel, T.,  Kozhurina-Platais, V.,  Demarque, P.: AJ {\bf 188}, 2894 (1999)
\bibitem{Sepinsky2009}  Sepinsky, J.F., Willems, B.,  Kalogera, V.,   Rasio, F.A.: ApJ {\bf 702}, 1387 (2009)
\bibitem{Sillsetal2005}  Sills, A., Adams, T.,  Davies, M. B.: MNRAS {\bf 358}, 716 (2005)
\bibitem{Sillsetal2001}  Sills, A.,  Faber, J. A.,  Lombardi, Jr., J. C.,  Rasio, F. A.,  Warren, A. R.: ApJ {\bf 548}, 323 (2001)
\bibitem{Soker2000}  Soker, N.: A\&A {\bf 357}, 557 (2000)
\bibitem{Tokovinin1997}  Tokovinin,  A. A.: A\&AS {\bf 124}, 75 (1997)
\bibitem{vandenBergetal2001}  van den Berg, M., Orosz, J. ,  Verbunt, F.,  Stassun, K.: A\&A {\bf 375}, 375 (2001)
\bibitem{Webbink1976} Webbink, R.F.: ApJ {\bf 209}, 829 (1976)
%\bibitem A.J. Whitehead, S.L.W. McMillan, S. Portegies Zwart, E. Vesperini, American Astronomical Society, AAS Meeting \#218, \#133.10  (2011)
\bibitem{WoodIvanova2011}  Woods, T. E.,  Ivanova, N.: ApJL {\bf  739}, 48 (2011)
\end{thebibliography}

==> refmcmillan.tex <==
\begin{thebibliography}{}

\bibitem{2003gnbs.book.....A}
Aarseth, S. J.: Gravitational N-Body Simulations, Cambridge
University Press (2003)

\bibitem{1973ApJ...179..885A}
Ahmad, A.,  Cohen, L.:  J. Comp. Phys. {\bf 12}, 289 (1973)

\bibitem{1962spss.book.....A}
Antonov, V. A.:  Vestn. Leningr. Gros. Univ. {\bf  7}, 135 (1962)

\bibitem{1996MNRAS.281..830B}
Bacon, D., Sigurdsson, S.,  Davies, M. B.:  MNRAS {\bf 281}, 830 (1996)

\bibitem{1986Natur.324..446B}
Barnes, J.,  Hut, P.:  Nature {\bf 324}, 446 (1986)

\bibitem{Bastian2013}
Bastian, N., Lamers, J. G. L. M, Longmore, S. N., Goodwin, S. P., de
Mink, S.,  Gieles, M.: MNRAS {\bf 436}, 2398 (2013)

\bibitem{2001MNRAS.325.1323B}
Baumgardt, H.:  MNRAS {\bf 325}, 1323 (2001)

\bibitem{2003MNRAS.340..227B}
Baumgardt, H.,  Makino, J.:  MNRAS {\bf 340}, 227
(2003)

\bibitem{Bekki2011}
Bekki, K.:  MNRAS {\bf 412}, 2241 (2011)

\bibitem{2008NewA...13..103B}
Belleman, R. G., B\'edorf, J.,  Portegies Zwart, S. F.: New
Astronomy {\bf 13}, 103 (2008)

\bibitem{1987ApJ...323..614B}
Benz, W.,  Hills, J. G.:  ApJ {\bf 323}, 614 (1987)

\bibitem{Berczik2011}
Berczik, P., Nitadori, 
K., Zhong, S., et al.: in Proc. 1st International Conference on
High-Performance Computing, HPC-UA, p.8 (2011)

\bibitem{1984MNRAS.208..493B}
Bettwieser, E.,  Sugimoto, D.:  MNRAS {\bf 208}, 493
(1984)

\bibitem{2008gady.book.....B}
Binney, J.,  Tremaine, S.:  Galactic Dynamics (2nd
Edition), Princeton University Press (2008)

\bibitem{Capuzzo-Dolcetta2012}
Capuzzo-Dolcetta, R., Spera, M.,  Punzo, D.:  Journal of Computational Physics {\bf 236}, 580  (2013)

\bibitem{Carretta2009a}
Carretta, E., Bragaglia, A., Gratton, et al.: 
%R. G., Lucatello, S., Catanzaro, G., Leone, F., Bellazzini, M., Claudi, R., D'Orazi, V., Momany, Y.,Ortolani, S., Pancino, E., Piotto, G., Recio-Blanco, A.,  Sabbi, E:
 A\&A {\bf 505}, 117 (2009a)

\bibitem{Carretta2009b}
Carretta, E., Bragaglia, A., Gratton, R.,  Lucatello, S.: 
A\&A {\bf 505}, 139 (2009b)

\bibitem{2008IAUS..246..151C}
Chatterjee, S., Fregeau, J. M.,  Rasio, F. A.: in Dynamical Evolution of Dense Stellar Systems, IAU Symp.
246, 151 (2008)

\bibitem{1990ApJ...351..121C}
Chernoff, D. F.,  Weinberg, M. D.:  ApJ {\bf 351}, 121
(1990)

\bibitem{1979ApJ...234.1036C}
Cohn, H.:  ApJ {\bf 234}, 1036 (1979)

\bibitem{1980ApJ...242..765C}
Cohn, H.:  ApJ {\bf 242}, 765 (1980)

\bibitem{Cohn1989}
Cohn, H., Hut, P.,  Wise, M.:  ApJ {\bf 342}, 814 (1989)

\bibitem{2001ApJ...550L..65V}
Cottrell, P. L.,  Da Costa, G. S.:  ApJ {\bf 245}, L79 (1981)

\bibitem{Ercole2008}
D'Ercole, A., Vesperini, E., D'Antona, F., McMillan, S. L. W.,
Recchi, S.:  MNRAS {\bf 391}, 825 (2008)

\bibitem{Ercole2010}
D'Ercole, A., D'Antona, F., Ventura, P., Vesperini, E.,  McMillan,
S. L. W.:  MNRAS {\bf 407}, 854 (2010)

\bibitem{deMink2009}
de Mink, S. E., Pols, O. R., Langer, N.,  Izzard, R. G.:  A\&A {\bf
507}, L1 (2009)

\bibitem{2007A&A...464.1029D}
Decressin, T., Meynet, G., Charbonnel, C., Prantzos, N.,  Ekstr\"om,
S.:  A\&A {\bf 464}, 1029 (2007)

\bibitem{Decressin2008}
Decressin, T., Baumgardt, H.,  Kroupa, P.:  A\&A {\bf 492}, 101 (2008)

\bibitem{2000ApJ...536L..39D}
Dehnen, W.:  ApJL {\bf 536}, L39 (2000)

\bibitem{2001A&AT...20...47D}
Deiters, S.,  Spurzem, R.: Astronomical and Astrophysical
Transactions {\bf 20}, 47 (2001)

\bibitem{1992ApJ...386..106D}
Drukier, G. A., Fahlman, G. G.,  Richer, H. B.:  ApJ {\bf 386}, 106 (1992)

\bibitem{1993PASJ...45..269E}
Ebisuzaki, T., Makino, J., Fukushige, T., Taiji, M.,  Sugimoto D.:
 PASJ {\bf 45}, 269 (1993)

\bibitem{1989ApJ...347..998E}
Eggleton, P. P., Fitchett, M. J.,  Tout, C. A.:  ApJ {\bf 347}, 998 (1989)

\bibitem{1999MNRAS.302...81E}
Einsel, C.,  Spurzem, R.:  MNRAS {\bf 302}, 81
(1999)

\bibitem{Fabian1975}
Fabian, A. C., Pringle, J. E.,  Rees, M. J.:  MNRAS {\bf 172}, 15P (1975)

\bibitem{2007ApJ...658.1047F}
Fregeau, J. M.,  Rasio, F. A.:  ApJ {\bf 658}, 1047 (2007)

\bibitem{2003ApJ...593..772F}
Fregeau, J. M., G\"urkan, M. A., Joshi, K.J.,  Rasio, F. A.:  ApJ {\bf
593}, 772 (2003)

\bibitem{2004MNRAS.352....1F}
Fregeau, J. M., Cheung, P., Portegies Zwart, S. F.,  Rasio,
F. A.:  MNRAS {\bf 352}, 1 (2004)

\bibitem{2001A&A...375..711F}
Freitag, M.,  Benz, W.:  A\&A {\bf 375}, 711 (2001)

\bibitem{2005MNRAS.358.1133F}
Freitag, M.,  Benz, W.:  MNRAS {\bf 358}, 1133 (2005)

\bibitem{2006MNRAS.368..121F}
Freitag, M., Rasio, F. A.,  Baumgardt, H.:  MNRAS {\bf 368}, 121 (2006)

\bibitem{2007PASJ...59.1095F}
Fujii, M., Iwasawa, M., Funato, Y.,  Makino, J.: 
PASJ {\bf 59}, 1095 (2007)

\bibitem{1995MNRAS.276..206F}
Fukushige, T.,  Heggie, D. C.:  MNRAS {\bf 276}, 206 (1995)

\bibitem{2000MNRAS.318..753F}
Fukushige, T.,  Heggie, D. C.:  MNRAS {\bf 318}, 753 (2000)

\bibitem{2009NewA...14..630G}
Gaburov, E., Harfst, S.,  Portegies Zwart, S. F.: New
Astronomy {\bf 14}, 630 (2009)

\bibitem{2008MNRAS.383L...5G}
Gaburov, E., Lombardi, J. C.,  Portegies Zwart S.: MNRAS {\bf 383},
L5 (2008)

\bibitem{1991ApJ...370..567G}
Gao, B., Goodman, J., Cohn, H.,  Murphy, B.:  ApJ {\bf 370}, 567 (1991)

\bibitem{1998MNRAS.298.1239G}
Giersz, M.:  MNRAS {\bf 298}, 1239 (1998)

\bibitem{2001MNRAS.324..218G}
Giersz, M.:  MNRAS {\bf 324}, 218 (2001)

\bibitem{2006MNRAS.371..484G}
Giersz, M.:  MNRAS {\bf 371}, 484 (2006)

\bibitem{Giersz1994}
Giersz, M.,  Heggie, D. C.:  MNRAS {\bf 268}, 257 (1994)

\bibitem{2009MNRAS.395.1173G}
Giersz, M.,  Heggie, D. C.:  MNRAS {\bf 395}, 1173 (2009)

\bibitem{Giersz2011}
Giersz, M.,  Heggie D. C.:  MNRAS {\bf 410}, 2698 (2011)

\bibitem{Giersz2013}
Giersz, M., Heggie, D.C., Hurley, J. R.,  Hypki, A.:  MNRAS {\bf
431}, 2184 (2013)

\bibitem{2003MNRAS.343..781G}
Giersz, M.,  Spurzem, R.:  MNRAS {\bf 343}, 781 (2003)

\bibitem{Goodman1987}
Goodman, J.:  ApJ {\bf 313}, 576 (1987)

\bibitem{1989Natur.339...40G}
Goodman, J.,  Hut, P.:  Nature {\bf 339}, 40 (1989)

\bibitem{Grindlay2006}
Grindlay, J. E., Portegies Zwart, S. F.  McMillan, S. L. W.:
Nature Physics {\bf 2}, 116 (2006)

\bibitem{2004ApJ...604..632G}
G\"urkan, M. A., Freitag, M.,  Rasio, F. A.:  ApJ {\bf 604}, 632 (2004)

\bibitem{2007astro.ph..3100H}
Hamada, T.,  Iitaka, T.: astro-ph/0703100 (2007)

\bibitem{1975MNRAS.173..729H}
Heggie, D. C.:  MNRAS {\bf 173}, 729 (1975)

\bibitem{1992MNRAS.257..513H}
Heggie, D. C.,  Aarseth, S. J.:  MNRAS {\bf 257}, 513 (1992)

\bibitem{2008MNRAS.389.1858H}
Heggie, D. C.,  Giersz, M.:  MNRAS {\bf 389}, 1858 (2008)

\bibitem{2003gmbp.book.....H}
Heggie, D. C.,  Hut, P.: The Gravitational Million-Body
Problem: A Multidisciplinary Approach to Star Cluster Dynamics, Cambridge University Press
(2003)

\bibitem{HM86}
Heggie, D. C.,  Mathieu R. D.: in The Use of Supercomputers in
Stellar Dynamics, LNP Vol. 267, Springer-Verlag, p. 13 (1986)

\bibitem{1965AnAp...28...62H}
H\'enon, M.:  Annales d'Astrophysique {\bf 28}, 62 (1965)

\bibitem{1973dses.conf..183H}
H\'enon, M.: in Saas-Fee Advanced Course 3: Dynamical Structure and
Evolution of Stellar Systems, Observatoire de Gen\'eve, p. 183 (1973)

\bibitem{1975AJ.....80..809H}
Hills, J. G.:  AJ {\bf 80}, 809 (1975)

\bibitem{1976ApL....17...87H}
Hills, J. G,  Day, C. A.:  ApJL {\bf 17}, 87 (1976)

\bibitem{2000MNRAS.315..543H}
Hurley, J. R., Pols, O. R.,  Tout, C. A.:  MNRAS {\bf 315}, 543 (2000)

\bibitem{2001MNRAS.323..630H}
Hurley, J. R., Tout, C. A., Aarseth, S. J.,  Pols, O. R.: 
MNRAS {\bf 323}, 630 (2001)

\bibitem{2002MNRAS.329..897H}
Hurley, J. R., Tout, C. A.,  Pols, O. R.:  MNRAS {\bf 329}, 897 (2002)

\bibitem{1983ApJ...268..319H}
Hut, P.,  Bahcall, J. N.:  ApJ {\bf 268}, 319 (1983)

\bibitem{1985ApJ...298..502H}
Hut, P.,  Inagaki, S.:  ApJ {\bf 298}, 502 (1985)

\bibitem{1988Natur.336...31H}
Hut, P., Makino, J.,  McMillan, S. L. W.:  Nature {\bf 336}, 31 (1988)

\bibitem{1985ApJ...292..339I}
Inagaki, S.,  Saslaw, W. C.:  ApJ {\bf 292}, 339 (1985)

\bibitem{2000ApJ...540..969J}
Joshi, K. J., Rasio, F. A.,  Portegies Zwart, S.:  ApJ {\bf 540}, 969 (2000)

\bibitem{2007PASA...24..103K}
Karakas, A.,  Lattanzio, J. C.: PASA {\bf 24},103 (2007)

\bibitem{2002MNRAS.334..310K}
Kim. E., Einsel, C., Lee, H-M., Spurzem, R.,  Lee, M. G.: 
MNRAS {\bf 334}, 310 (2002)

\bibitem{2004MNRAS.351..220K}
Kim. E., Lee, H-M.,  Spurzem, R.:  MNRAS {\bf 351}, 220 (2004)

\bibitem{1966AJ.....71...64K}
King, I. R.:  AJ {\bf 71}, 64 (1966)

\bibitem{2001MNRAS.322..231K}
Kroupa, P.:  MNRAS {\bf 322}, 231 (2001)

\bibitem{2006MNRAS.371L..45K}
Kupi, G., Amaro-Seoane, P.,  Spurzem, R.:  MNRAS {\bf 371}, L45 (2006)

\bibitem{2005A&A...429..173L}
Lamers, H. J. G. L. M., Gieles, M.,  Portegies Zwart, S. F.: 
A\&A {\bf 429}, 173 (2005)

\bibitem{2003MNRAS.345..762L}
Lombardi, J. C., Thrall, A. P., Deneva, J. S., Fleming, S. W., 
Grabowski PE.:  MNRAS {\bf 345}, 762 (2003)

\bibitem{1980MNRAS.191..483L}
Lynden-Bell, D.,  Eggleton, P. P.:  MNRAS {\bf 191}, 483 (1980)

\bibitem{1968MNRAS.138..495L}
Lynden-Bell, D.,  Wood, R.:  MNRAS {\bf 138}, 495 (1968)

\bibitem{Makino1996}
Makino, J.: ApJ {\bf 471}, 796 (1996)

\bibitem{2005astro.ph..9278M}
Makino, J.: astro-ph/0509278 (2005)

\bibitem{1992PASJ...44..141M}
Makino, J.,  Aarseth, S. J.:  PASJ {\bf 44}, 141 (1992)

\bibitem{2006NewA...12..124M}
Makino, J., Hut, P., Kaplan, M.,  {Sayg{\i}n}, H.: New Astronomy {\bf 12}, 124 (2006)

\bibitem{1986LNP...267..156M}
McMillan, S. L. W.: in The Use of Supercomputers in Stellar
Dynamics, LNP Vol. 267, Springer-Verlag, p. 156 (1986)

\bibitem{1993ApJ...414..200M}
McMillan, S. L. W.,  Aarseth, S. J.:  ApJ {\bf 414}, 200 (1993)

\bibitem{1990ApJ...362..522M}
McMillan, S. L. W., Hut, P.,  Makino, J.:  ApJ {\bf 362}, 522 (1990)

\bibitem{1991ApJ...372..111M}
McMillan, S. L. W., Hut, P., Makino, J.: ApJ {\bf 372}, 111 (1991)

\bibitem{McMillan2011}
McMillan, S., Portegies Zwart, S., van Elteren, A.,  Whitehead,
A.: in Advances in Computational Astrophysics: methods, tools
and outcomes, ASPC 435, p.129 (2012)

\bibitem{2008MmSAI..79..623M}
Milone, A. P., Piotto, G., Bedin, L. R.,  Sarajedini, A.: MmSAI {\bf 79}, 623 (2008)

\bibitem{1999MNRAS.310.1147M}
Moore, B., Quinn, T., Governato, F., Stadel, J.,  Lake, G.: 
MNRAS {\bf 310}, 1147 (1999)

%\bibitem{}
%Nitadori, K., Makino, J.,  Hut, P. 2006, New Astronomy, 12, 169

\bibitem{2008NewA...13..498N}
Nitadori, K.,  Makino, J.:  New Astronomy {\bf 13}, 498 (2008)

\bibitem{2012MNRAS.424..545N}
Nitadori, K.,  Aarseth, S. J.:  MNRAS {\bf 424}, 545 (2012)

\bibitem{Pelupessy2012}
Pelupessy, F. I.,  Portegies Zwart, S.:  MNRAS {\bf 420}, 1503 (2012)

\bibitem{Pelupessy2013}
Pelupessy, F. I., van Elteren, A., de Vries, N., McMillan, S.L.W., 
Drost, N.,  Portegies Zwart, S.F.: A\&A {\bf 557}, A84 (2013)

\bibitem{2005ApJ...621..777P}
Piotto, G., Villanova, S., Bedin, L. R., Gratton, R., Cassisi, S., et
al.:  ApJ {\bf 621}, 777 (2005)

\bibitem{2008MmSAI..79..334P}
Piotto, G.:  MmSAI {\bf 79}, 334 (2008)

\bibitem{1911MNRAS..71..460P}
Plummer, H. C.:  MNRAS {\bf 71}, 460 (1911)

\bibitem{2002ApJ...576..899P}
Portegies Zwart, S. F.,  McMillan, S. L. W.:  ApJ {\bf 576}, 899 (2002)

\bibitem{1999CeMDA..73..179P}
Portegies Zwart, S. F.,  Takahashi, K.: Celestial Mechanics and
Dynamical Astronomy {\bf 73}, 179 (1999)

\bibitem{1996A&A...309..179P}
Portegies Zwart, S. F.,  Verbunt, F.:  A\&A {\bf 309}, 179 (1996)

\bibitem{1999A&A...348..117P}
Portegies Zwart, S. F., Makino, J., McMillan, S. L. W.,  Hut, P.:  A\&A {\bf 348}, 117 (1999)

\bibitem{2001MNRAS.321..199P}
Portegies Zwart, S. F., McMillan, S. L. W., Hut, P.,  Makino,
J.:  MNRAS {\bf 321}, 199 (2001)

\bibitem{2009NewA...14..369P}
Portegies Zwart, S. F., McMillan, S. L. W., Harfst, S., Groen, D.,
Fujii, M., et al.:  New Astronomy {\bf  14}, 369 (2009)

\bibitem{2007NewA...12..641P}
Portegies Zwart, S. F., Belleman, R. G.,  Geldof, P. M.:  New Astronomy {\bf  12}, 641 (2007)

\bibitem{Zwart2013}
Portegies Zwart, S., McMillan, S. L. W., van Elteren, E., Pelupessy,
I.,  de Vries, N.: Computer Physics Communications {\bf 184}, 456 (2013)

\bibitem{2006A&A...458..135P}
Prantzos, N.,  Charbonnel, C.:  A\&A {\bf 458}, 135 (2006)

\bibitem{1996NewA....1..255Q}
Quinlan, G. D.:  New Astronomy {\bf 1}, 255 (1996)

\bibitem{Renzini2008}
Renzini, A.:  MNRAS {\bf 391}, 354 (2008)

\bibitem{1985IAUS..113..373S}
Shapiro, S. L.: in Dynamics of Star Clusters,
IAU Symp. 113, p. 373 (1985)

\bibitem{1975IAUS...69....3S}
Spitzer, L.:  in Dynamics of the Solar Systems,
IAU Symp. 69, p. 3 (1975)

\bibitem{1987degc.book.....S}
Spitzer, L.: Dynamical evolution of globular clusters, Princeton University Press (1987)

\bibitem{1969ApJ...158L.139S}
Spitzer, L. J.: ApJL {\bf 158}, 139 (1989)

\bibitem{1971ApJ...164..399S}
Spitzer, L. J  Hart, M. H.:  ApJ {\bf 164}, 399 (1971)

\bibitem{1999JCoAM.109..407S}
Spurzem, R.: Journal of Computational and Applied Mathematics
{\bf 109}, 407 (1999)

\bibitem{Spurzem2008}
Spurzem, R., Berentzen, I., Berczik, P., Merritt, D., Amaro-Seoane,
P., Harfst, S.,  Gualandris, A.: in The Cambridge N-Body
Lectures, LNP Vol. 760, Springer-Verlag, p. 377 (2008)

\bibitem{1982AcA....32...63S}
Stodolkiewicz, J. S.: Acta Astron. {\bf 32}, 63 (1982)

\bibitem{1986AcA....36...19S}
Stodolkiewicz, J. S.: Acta Astron. {\bf 36}, 19 (1986)

\bibitem{1996PASJ...48..691T}
Takahashi, K.:  PASJ {\bf 48}, 691 (1996)

\bibitem{1997PASJ...49..547T}
Takahashi, K.:  PASJ {\bf 49}, 547 (1997)

\bibitem{1998ApJ...503L..49T}
Takahashi, K.,  Portegies Zwart, S. F.:  ApJL {\bf 503}, 49 (1998)

\bibitem{2000ApJ...535..759T}
Takahashi, K.,  Portegies Zwart, S. F.:  ApJ {\bf 535}, 759 (2000)

\bibitem{Tanikawa2012}
Tanikawa, A., Hut, P.,  Makino, J.: New Astronomy {\bf  17}, 272 (2012)

\bibitem{Ventura2001}
Ventura, P., D'Antona, F., Mazzitelli, I.,  Gratton, R.:  ApJL {\bf
550}, 65 (2001)

\bibitem{Vesperini2011}
Vesperini, E., McMillan, S. L. W., D'Antona, F.,  D'Ercole, A.:
MNRAS {\bf 416}, 355 (2011)

\bibitem{Vesperini2013}
Vesperini, E., McMillan, S. L. W., D'Antona, F.,  D'Ercole, A.:
MNRAS {\bf 429}, 1913 (2013)

\bibitem{2009ApJ...698..615V}
Vesperini, E., McMillan, S. L. W.,  Portegies Zwart, S.: ApJ {\bf
698}, 615 (2009)

\bibitem{Wang2013}
Wang, L., Nitadori, K., Spurzem, R., Berczik, P.,  Aarseth S.J.:
in prep. (2014)

\bibitem{Whitehead2013}
Whitehead, A., McMillan, S. L. W., Vesperini, E.,  Portegies Zwart,
S.: ApJ {\bf 778}, 118 (2013)

\end{thebibliography}

==> refmomany.tex <==
\begin{thebibliography}{79}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem{Aparicio2001c}
{Aparicio}, A., {Carrera}, R.,  {Mart{\'{\i}}nez-Delgado}, D.:  AJ {\bf 122},
  2524 (2001)

\bibitem{Beccari2008}
{Beccari}, G., {Pulone}, L., {Ferraro}, F.~R., {et~al.}: MemSAI {\bf 79}, 360 (2008)

\bibitem{Beccari2011}
{Beccari}, G., {Sollima}, A., {Ferraro}, F.~R., {et~al.}: ApJL {\bf 737}, 3 (2011)

\bibitem{Belokurov2006c}
{Belokurov}, V., {Zucker}, D.~B., {Evans}, N.~W., {et~al.}: ApJL {\bf 647},
  111 (2006)

\bibitem{Bernard2009c}
{Bernard}, E.~J., {Monelli}, M., {Gallart}, C., {et~al.}: ApJ {\bf 699}, 1742 (2009)

\bibitem{Blumenthal1984d}
{Blumenthal}, G.~R., {Faber}, S.~M., {Primack}, J.~R.,  {Rees}, M.~J.:
 Nature {\bf 311}, 517 (1984)

\bibitem{Bono2010e}
{Bono}, G., {Stetson}, P.~B., {Walker}, A.~R., {et~al.}: PASP {\bf 122}, 651 (2010)

\bibitem{Brown2008}
{Brown}, T.~M., {Beaton}, R., {Chiba}, M., {et~al.}: ApJL {\bf 685}, 121 (2008)

\bibitem{Carrera2002e}
{Carrera}, R., {Aparicio}, A., {Mart{\'{\i}}nez-Delgado}, D., \&
  {Alonso-Garc{\'{\i}}a}, J.: AJ {\bf 123}, 3199 (2002)

\bibitem{Carretta2009f}
{Carretta}, E., {Bragaglia}, A., {Gratton}, R.~G., {et~al.}: A\&A {\bf 505},
  117 (2009)

\bibitem{Clarkson2011c}
{Clarkson}, W.~I., {Sahu}, K.~C., {Anderson}, J., {et~al.}: ApJ {\bf 735}, 37 (2011)

\bibitem{Cohen2012b}
{Cohen}, R.~E.  {Sarajedini}, A.: {\bf 419}, 342 (2012)

\bibitem{Davies2004a}
{Davies}, M.~B., {Piotto}, G.,  {de Angeli}, F.: {\bf 349}, 129 (2004)

\bibitem{2006A&A...459..489D}
{de Marchi}, F., {de Angeli}, F., {Piotto}, G., {Carraro}, G.,  {Davies},
  M.~B.: A\&A {\bf 459}, 489 (2006)

\bibitem{Ferraro1997e}
{Ferraro}, F.~R., {Paltrinieri}, B., {Fusi Pecci}, F., {et~al.}: A\&A {\bf 324}, 915 (1997)

\bibitem{Ferraro1999a}
{Ferraro}, F.~R., {Paltrinieri}, B., {Rood}, R.~T.,  {Dorman}, B.: ApJ {\bf 
  522}, 983 (1999)

\bibitem{Ferraro2006a}
{Ferraro}, F.~R., {Sollima}, A., {Rood}, R.~T., {et~al.}: ApJ {\bf 638}, 433 (2006)

\bibitem{Fiorentino2006a}
{Fiorentino}, G., {Limongi}, M., {Caputo}, F.,  {Marconi}, M.: A\&A {\bf 460}, 155 (2006)

\bibitem{Fiorentino2012f}
{Fiorentino}, G.  {Monelli}, M.: A\&A {\bf 540}, A102 (2012)

\bibitem{Fiorentino2012b}
{Fiorentino}, G., {Stetson}, P.~B., {Monelli}, M., {et~al.}: ApJL {\bf 759},
  12 (2012)

\bibitem{FusiPecci1992}
{Fusi Pecci}, F., {Ferraro}, F.~R., {Corsi}, C.~E., {Cacciari}, C., \&
  {Buonanno}, R.: AJ {\bf 104}, 1831 (1992)

\bibitem{Gallart1999c}
{Gallart}, C., {Freedman}, W.~L., {Mateo}, M., {et~al.}: ApJ {\bf 514}, 665 (1999)

\bibitem{Gilmore2007cm}
{Gilmore}, G., {Wilkinson}, M.~I., {Wyse}, R.~F.~G., {et~al.}: ApJ {\bf 663},
  948 (2007)

\bibitem{Girardi2005}
{Girardi}, L., {Groenewegen}, M.~A.~T., {Hatziminaoglou}, E.,  {da Costa}, L.: A\&A {\bf 436}, 895 (2005)

\bibitem{Held2005}
{Held}, E.~V.: , in IAU Colloq. 198: Near-fields cosmology with dwarf
  elliptical galaxies, p. 11 (2005)

\bibitem{Held2000}
{Held}, E.~V., {Saviane}, I., {Momany}, Y.,  {Carraro}, G.: ApJL {\bf 530},
  85 (2000)

\bibitem{Hills1976d}
{Hills}, J.~G.  {Day}, C.~A.:  ApJL {\bf 17}, 87 (1976)

\bibitem{Holtzman2006d}
{Holtzman}, J.~A., {Afonso}, C.,  {Dolphin}, A.: ApJS {\bf 166}, 534 (2006)

\bibitem{Hurley-Keller1998}
{Hurley-Keller}, D., {Mateo}, M.,  {Nemec}, J.: AJ {\bf 115}, 1840 (1998)

\bibitem{Keller2012am}
{Keller}, S.~C., {Skymapper Team},  {Aegis Team}: in Galactic Archaeology:
  Near-Field Cosmology and the Formation of the Milky Way, ASPC 458, p. 409 (2012)

\bibitem{Lanzoni2007}
{Lanzoni}, B., {Dalessandro}, E., {Ferraro}, F.~R., {et~al.}:
 ApJ {\bf 663}, 267 (2007a)

\bibitem{Lanzoni2007a}
{Lanzoni}, B., {Sanna}, N., {Ferraro}, F.~R., {et~al.}:
  ApJ {\bf 663}, 1040 (2007b)

\bibitem{Lee2003u}
{Lee}, M.~G., {Park}, H.~S., {Park}, J.-H., {et~al.}: AJ {\bf 126}, 2840 (2003)

\bibitem{Mandushev1997}
{Mandushev}, G.~I., {Fahlman}, G.~G., {Richer}, H.~B.,  {Thompson}, I.~B.: AJ {\bf 114}, 1060 (1997)

\bibitem{Mapelli2009d}
{Mapelli}, M., {Ripamonti}, E., {Battaglia}, G., {et~al.}: MNRAS {\bf 396},
  1771 (2009)

\bibitem{Mapelli2007b}
{Mapelli}, M., {Ripamonti}, E., {Tolstoy}, E., {et~al.}: MNRAS {\bf 380}, 1127 (2007)

\bibitem{Mapelli2004}
{Mapelli}, M., {Sigurdsson}, S., {Colpi}, M., {et~al.}: ApJL {\bf 605}, 29 (2004)

\bibitem{Mapelli2006c}
{Mapelli}, M., {Sigurdsson}, S., {Ferraro}, F.~R., {et~al.}: MNRAS {\bf  373},
  361 (2006)

\bibitem{Marin-Franch2009}
{Mar{\'{\i}}n-Franch}, A., {Aparicio}, A., {Piotto}, G., {et~al.}: ApJ {\bf 694}, 1498 (2009)

\bibitem{Martin2008}
{Martin}, N.~F., {Coleman}, M.~G., {De Jong}, J.~T.~A., {et~al.}: ApJL {\bf 672}, 13 (2008)

\bibitem{Mateo1995c}
{Mateo}, M., {Fischer}, P.,  {Krzeminski}, W.:  AJ {\bf 110}, 2166 (1995)

\bibitem{Mateo1998d}
{Mateo}, M., {Hurley-Keller}, D.,  {Nemec}, J.:  AJ {\bf 115}, 1856 (1998)

\bibitem{Mateo1991a}
{Mateo}, M., {Nemec}, J., {Irwin}, M.,  {McMahon}, R.: AJ {\bf 101}, 892 (1991)

\bibitem{Mateo1998}
{Mateo}, M.~L.:  ARA\&A {\bf 36}, 435 (1998)

\bibitem{McConnachie2012a}
{McConnachie}, A.~W.: AJ {\bf 144}, 4 (2012)

\bibitem{McCrea1964a}
{McCrea}, W.~H.: MNRAS {\bf 128}, 147 (1964)

\bibitem{Milone2013d}
{Milone}, A.~P., {Marino}, A.~F., {Piotto}, G., {et~al.}: ApJ {\bf 767}, 120 (2013)

\bibitem{Misgeld2011}
{Misgeld}, I.  {Hilker}, M.: MNRAS {\bf 414}, 3699 (2011)

\bibitem{Momany2003b}
{Momany}, Y., {Cassisi}, S., {Piotto}, G., {et~al.}: A\&A {\bf 407}, 303 (2003)

\bibitem{Momany2007}
{Momany}, Y., {Held}, E.~V., {Saviane}, I., {et~al.}: A\&A {\bf 468}, 973 (2007)

\bibitem{Monaco2003a}
{Monaco}, L., {Bellazzini}, M., {Ferraro}, F.~R.,  {Pancino}, E.:  ApJL {\bf 597}, 25 (2003)

\bibitem{Monelli2012}
{Monelli}, M., {Cassisi}, S., {Mapelli}, M., {et~al.}: ApJ {\bf 744}, 157 (2012)

\bibitem{Monelli2010a}
{Monelli}, M., {Hidalgo}, S.~L., {Stetson}, P.~B., {et~al.}: ApJ {\bf 720},
  1225 (2010)

\bibitem{Monkman2006}
{Monkman}, E., {Sills}, A., {Howell}, J., {et~al.}: ApJ {\bf 650}, 195 (2006)

\bibitem{Niederste-Ostholt2009}
{Niederste-Ostholt}, M., {Belokurov}, V., {Evans}, N.~W., {et~al.}:
MNRAS  {\bf 398}, 1771 (2009)

\bibitem{Piotto2004c}
{Piotto}, G., {De Angeli}, F., {King}, I.~R., {et~al.}: ApJL {\bf 604}, 109 (2004)

\bibitem{Piotto2002}
{Piotto}, G., {de Angeli}, F., {Recio Blanco}, A., {et~al.}: in
  Observed HR
  Diagrams and Stellar Evolution, ASPC 274, p. 282 (2002)

\bibitem{Poretti1999}
{Poretti}, E.:  A\&A {\bf 343}, 385 (1999)

\bibitem{Poretti2008}
{Poretti}, E., {Clementini}, G., {Held}, E.~V., {et~al.}: ApJ {\bf 685}, 947 (2008)

\bibitem{Preston2000e}
{Preston}, G.~W.  {Sneden}, C.: AJ {\bf 120}, 1014 (2000)

\bibitem{Pritzl2002c}
{Pritzl}, B.~J., {Armandroff}, T.~E., {Jacoby}, G.~H.,  {Da Costa}, G.~S.: AJ {\bf 124}, 1464 (2002)

\bibitem{Renzini2013}
{Renzini}, A.: MmSAI {\bf
84}, 162 
(2013)

\bibitem{Renzini1988}
{Renzini}, A.  {Fusi Pecci}, F.: ARA\&A {\bf 26}, 199 (1988)

\bibitem{Renzini1977b}
{Renzini}, A., {Mengel}, J.~G.,  {Sweigart}, A.~V.:  A\&A {\bf 56}, 369 (1977)

\bibitem{Rizzi2003e}
{Rizzi}, L., {Held}, E.~V., {Bertelli}, G.,  {Saviane}, I.:
  ApJL {\bf 589}, 85 (2003a)

\bibitem{Rizzi2003}
{Rizzi}, L., {Held}, E.~V., {Momany}, Y., {et~al.}: MmSAI {\bf 74}, 510 (2003b)

\bibitem{YoSandage1953}
{Sandage}, A.~R.: AJ {\bf 58}, 61 (1953)

\bibitem{Santana2012}
{Santana}, F.~A., {Mu{\~n}oz}, R.~R., {Geha}, M., {et~al.}: in
  Galactic
  Archaeology: Near-Field Cosmology and the Formation of the Milky Way, ASPC 458, p. 339 (2012)

\bibitem{Saviane2000d}
{Saviane}, I., {Held}, E.~V.,  {Bertelli}, G.: A\&A {\bf 355}, 56 (2000)

\bibitem{Saviane2003}
{Saviane}, I., {Rosenberg}, A., {Aparicio}, A.,  {Piotto}, G.: in
  New Horizons
  in Globular Cluster, ASPC 296, p. 402 (2003)

\bibitem{Sills2009a}
{Sills}, A., {Karakas}, A.,  {Lattanzio}, J.: ApJ {\bf 692}, 1411 (2009)

\bibitem{Sollima2008c}
{Sollima}, A., {Lanzoni}, B., {Beccari}, G., {Ferraro}, F.~R.,  {Fusi Pecci},
  F.: A\&A {\bf 481}, 701 (2008)

\bibitem{Stryker1993}
{Stryker}, L.~L.: PASP {\bf 105}, 1081 (1993)

\bibitem{White1978e}
{White}, S.~D.~M.  {Rees}, M.~J.: MNRAS {\bf 183}, 341 (1978)

\bibitem{Willman2005a}
{Willman}, B., {Dalcanton}, J.~J., {Martinez-Delgado}, D., {et~al.}:
  ApJL {\bf 626}, 85 (2005)

\bibitem{Willman2012}
{Willman}, B.  {Strader}, J.: AJ {\bf 144}, 76 (2012)

\bibitem{Zaggia1997}
{Zaggia}, S.~R., {Piotto}, G.,  {Capaccioli}, M.: A\&A {\bf 327}, 1004 (1997)

\bibitem{Zhao2012bl}
{Zhao}, Z., {Okamoto}, S., {Arimoto}, N., {Aoki}, W.,  {Kodama}, T.: in
  Galactic
  Archaeology: Near-Field Cosmology and the Formation of the Milky Way, ASPC 458,  p. 349 (2012)

\bibitem{Zinn1976}
{Zinn}, R.  {Dahn}, C.~C.: AJ {\bf 81}, 527 (1976)

\end{thebibliography}


==> refperets.tex <==
\begin{thebibliography}{}

\bibitem{aba+13}
{Abate}, C.,  {Pols}, O.~R.,  {Izzard}, R.~G.,  {Mohamed}, S.~S.,    {de Mink}
  S.~E.: A\&A {\bf  552}, A26 (2013)

\bibitem{ant+12}
{Antonini}, F.,  {Perets}, H.~B.:   ApJ {\bf 757}, 27 (2012)

\bibitem{aur+90}
{Auriere}, M.,  {Lauzeral}, C.,    {Ortolani}, S.:   Nature {\bf 344}, 638 (1990)

\bibitem{benz+87}
{Benz}, W.,  {Hills}, J.~G.:   ApJ {\bf 323}, 614 (1987)

\bibitem{car+05}
{Carney}, B.~W.,  {Latham}, D.~W.,    {Laird}, J.~B.:   AJ {\bf 129}, 466 (2005)

\bibitem{car+01}
{Carney}, B.~W.,  {Latham}, D.~W.,  {Laird}, J.~B.,  {Grant}, C.~E.,    {Morse},
  J.~A.:  AJ {\bf 122}, 3419 (2001)

\bibitem{cha+13}
{Chatterjee}, S.,  {Rasio}, F.~A.,  {Sills}, A.,    {Glebbeek}, E.: ApJ {\bf 777}, 106 (2013)

\bibitem{che+08}
{Chen}, X.,  {Han}, Z.:  MNRAS {\bf 387}, 1416 (2008)

\bibitem{cla+11}
{Clarkson}, W.~I.,  {Sahu}, K.~C.,  {Anderson}, J.,  {Rich}, R.~M.,  {Smith}, T.~E.,
   {Brown}, T.~M.,  {Bond}, H.~E.,  {Livio}, M.,  {Minniti}, D.,  {Renzini}, A.,
  {Zoccali}, M.:  ApJ {\bf 735}, 37 (2011)

\bibitem{dav95}
{Davies}, M.~B.: MNRAS {\bf 276}, 887 (1995)

\bibitem{der+13}
{Dermine}, T.,  {Izzard}, R.~G.,  {Jorissen}, A.,    {Van Winckel}, H.:
  A\&A {\bf  551}, A50 (2013)

\bibitem{egg06}
{Eggleton}, P.:   {Evolutionary Processes in Binary and Multiple Stars}, Cambridge University Press (2006)

\bibitem{2001EK}
{Eggleton}, P.~P.,  {Kiseleva-Eggleton}, L.:   ApJ {\bf 562}, 1012 (2001)

\bibitem{2006EK}
{Eggleton}, P.~P.,  {Kisseleva-Eggleton}, L.:  Ap\&SS {\bf 304}, 75 (2006)

\bibitem{2007FT}
{Fabrycky}, D.,  {Tremaine}, S.: ApJ {\bf 669}, 1298 (2007)

\bibitem{fer+12}
{Ferraro}, F.~R.,  {Lanzoni}, B.,  {Dalessandro}, E.,  {Beccari}, G.,  {Pasquato}
  M.,  {Miocchi}, P.,  {Rood}, R.~T.,  {Sigurdsson}, S.,  {Sills}, A.,  {Vesperini}
  E.,  {Mapelli}, M.,  {Contreras}, R.,  {Sanna}, N.,    {Mucciarelli}, A.:
  Nature {\bf 492}, 393 (2012)

\bibitem{fer+97}
{Ferraro}, F.~R.,  {Paltrinieri}, B.,  {Fusi Pecci}, F.,  {Cacciari}, C.,  {Dorman}
  B.,  {Rood}, R.~T.,  {Buonanno}, R.,  {Corsi}, C.~E.,  {Burgarella}, D.,
  {Laget}, M.: A\&A {\bf 324}, 915 (1997)

\bibitem{fre+04}
{Fregeau}, J.~M.,  {Cheung}, P.,  {Portegies Zwart}, S.~F.,    {Rasio}, F.~A.:
   MNRAS {\bf 352}, 1 (2004)

\bibitem{gel+13}
{Geller}, A.~M.,  {Hurley}, J.~R.,    {Mathieu}, R.~D.: AJ {\bf 145}, 8 (2013)

\bibitem{gel+12}
{Geller}, A.~M.,  {Mathieu}, R.~D.: AJ {\bf 144}, 54 (2012)

\bibitem{gel+08}
{Geller}, A.~M.,  {Mathieu}, R.~D.,  {Harris}, H.~C.,    {McClure}, R.~D.: 
  AJ {\bf 135}, 2264 (2008)

\bibitem{ham+13}
{Hamers}, A.~S.,  {Pols}, O.~R.,  {Claeys}, J.~S.~W.,    {Nelemans}, G.:
  MNRAS {\bf 430}, 2262 (2013)

\bibitem{1968H}
{Harrington}, R.~S.:  AJ {\bf 73}, 190 (1968)

\bibitem{hil+76}
{Hills}, J.~G.,  {Day}, C.~A.: ApJL {\bf 17}, 87 (1976)

\bibitem{hur+05}
{Hurley}, J.~R.,  {Pols}, O.~R.,  {Aarseth}, S.~J.,    {Tout}, C.~A.:
  MNRAS {\bf 363}, 293 (2005)

\bibitem{hyp+13}
{Hypki}, A.,  {Giersz}, M.: MNRAS {\bf 429}, 1221 (2013)

\bibitem{2008I}
{Ivanova}, N.: in Multiple Stars Across the H-R Diagram {Population of Dynamically Formed
  Triples in Dense Stellar Systems}, Springer-Verlag, 
p.~101 (2008)

\bibitem{jor+98}
{Jorissen}, A.,  {Van Eck}, S.,  {Mayor}, M.,    {Udry}, S.:  A\&A {\bf 332}, 877 (1998)

\bibitem{kat+13}
{Katz}, B.,  {Dong}, S.:  arXiv:1211.4584 (2012)

\bibitem{kip+94}
{Kippenhahn}, R.,  {Weigert}, A.: {Stellar Structure and Evolution}, Springer-Verlag (1994)

\bibitem{1998KEM}
{Kiseleva}, L.~G.,  {Eggleton}, P.~P.,    {Mikkola}, S.:   MNRAS {\bf 300}, 292 (1998)

\bibitem{1962K}
{Kozai}, Y.:   AJ {\bf 67}, 591 (1962)

\bibitem{lan+97}
{Landsman}, W.,  {Aparicio}, J.,  {Bergeron}, P.,  {Di Stefano}, R.,    {Stecher}
  T.~P.:  ApJL {\bf 481}, 93 (1997)

\bibitem{lat+07}
{Latham}, D.~W.: Highlights of Astronomy {\bf 14}, 444 (2007)

\bibitem{lei+13}
{Leigh}, N.,  {Knigge}, C.,  {Sills}, A.,  {Perets}, H.~B.,  {Sarajedini}, A.,
  {Glebbeek}, E.: MNRAS {\bf 428}, 897 (2013)

\bibitem{lei+11}
{Leigh}, N.,  {Sills}, A.: MNRAS {\bf 410}, 2370 (2011)

\bibitem{leo89}
{Leonard}, P.~J.~T.: AJ {\bf 98}, 217 (1989)

\bibitem{leo96}
{Leonard}, P.~J.~T.: ApJ {\bf 470}, 521 (1996)

\bibitem{leo+91}
{Leonard}, P.~J.~T.,  {Fahlman}, G.~G.: AJ {\bf 102}, 994 (1991)

\bibitem{leo+92}
{Leonard}, P.~J.~T.,  {Linnell}, A.~P.: AJ {\bf 103}, 1928 (1992)

\bibitem{leo+95}
{Leonard}, P.~J.~T.,  {Livio}, M.: ApJL {\bf 447}, 121 (1995)

\bibitem{1962L}
{Lidov}, M.~L.: Planetary \& Sp. Sci. {\bf 9}, 719 (1962)

\bibitem{lov+10}
{Lovisi}, L.,  {Mucciarelli}, A.,  {Ferraro}, F.~R.,  {Lucatello}, S.,  {Lanzoni}
  B.,  {Dalessandro}, E.,  {Beccari}, G.,  {Rood}, R.~T.,  {Sills}, A.,  {Fusi
  Pecci}, F.,  {Gratton}, R.,    {Piotto}, G.: ApJL {\bf 719}, 121 (2010)

\bibitem{lov+13}
{Lovisi}, L.,  {Mucciarelli}, A.,  {Lanzoni}, B.,  {Ferraro}, F.~R.,
  {Dalessandro}, E.:  MmSAI {\bf 84}, 232 (2013)
  
\bibitem{map+04}
{Mapelli}, M.,  {Sigurdsson}, S.,  {Colpi}, M.,  {Ferraro}, F.~R.,  {Possenti}, A.,
  {Rood}, R.~T.,  {Sills}, A.,    {Beccari}, G.: ApJL {\bf 605}, 29 (2004)

\bibitem{mat+90}
{Mateo}, M.,  {Harris}, H.~C.,  {Nemec}, J.,    {Olszewski}, E.~W.: AJ {\bf
  100}, 469 (1990)

\bibitem{mat+86}
{Mathieu}, R.~D.,  {Latham}, D.~W.:   AJ {\bf 92}, 1364 (1986)

\bibitem{1979MS}
{Mazeh}, T.,  {Shaham}, J.:   A\&A {\bf 77}, 145 (1979)

\bibitem{mcc+90}
{McClure}, R.~D.,  {Woodsworth}, A.~W.: ApJ {\bf 352}, 709 (1990)

\bibitem{mcc64}
{McCrea}, W.~H.:  MNRAS {\bf 128}, 147 (1964a)

\bibitem{mcc+64}
{McCrea}, W.~H.: MNRAS {\bf 128}, 335 (1964b)

\bibitem{mer+96}
{Mermilliod}, J.-C.,  {Mayor}, M.: in Cool Stars, Stellar Systems, and the Sun, ASPC 109,
p.~373 (1996)

\bibitem{nem+95}
{Nemec}, J.~M.,  {Mateo}, M.,  {Burke}, M.,    {Olszewski}, E.~W.: AJ {\bf 110},
  1186 (1995)

\bibitem{per09a}
{Perets}, H.~B.: ApJ {\bf 698}, 1330 (2009)

\bibitem{per11}
{Perets}, H.~B.: ApJL {\bf 727}, 3 (2011)

\bibitem{per+09}
{Perets}, H.~B.,  {Fabrycky}, D.~C.:   ApJ {\bf 697}, 1048 (2009)

\bibitem{per+12}
{Perets}, H.~B.,  {Kratter}, K.~M.: ApJ {\bf 760}, 99 (2012)

\bibitem{rag+10}
{Raghavan}, D.,  {McAlister}, H.~A.,  {Henry}, T.~J.,  {Latham}, D.~W.,  {Marcy}
  G.~W.,  {Mason}, B.~D.,  {Gies}, D.~R.,  {White}, R.~J.,    {ten Brummelaar}
  T.~A.: ApJS {\bf 190}, 1 (2010)

\bibitem{ruc+00}
{Rucinski}, S.~M.: AJ {\bf 120}, 319 (2000)

\bibitem{sha+97}
{Shara}, M.~M.,  {Saffer}, R.~A.,    {Livio}, M.:  ApJL {\bf 489}, 59 (1997)

\bibitem{2006T}
{Tokovinin}, A.,  {Thomas}, S.,  {Sterzik}, M.,    {Udry}, S.:   A\&A {\bf 450},
  681 (2006)

\bibitem{wel+07}
{Weldrake}, D.~T.~F.,  {Sackett}, P.~D.,    {Bridges}, T.~J.: AJ {\bf 133},
  1447 (2007)

\bibitem{wel+04}
{Weldrake}, D.~T.~F.,  {Sackett}, P.~D.,  {Bridges}, T.~J.,    {Freeman}, K.~C.: AJ {\bf 128}, 736 (2004)

\end{thebibliography}


==> refpreston.tex <==
\begin{thebibliography}{999}%
\bibitem{ba11} Balona, L. A.  Dziembowski, W. A.: MNRAS  \textbf{417}, 591 (2011)
\bibitem{be09} Beccari, G., et al.: MmSAI, \textbf{80}, 107 (2009)
\bibitem{bee88} Beers, T. C., Prestoln, G. W.,  Shectman, S. A.: ApJS  \textbf{67}, 461 (1988)
\bibitem{bee92} Beers, T. C., Preston, G. W.,  Shectman, S. A.: AJ \textbf{103}, 1987 (1992)
\bibitem{bee96} Beers, T. C., et. al.: ApJS  \textbf{103}, 433 (1996)
\bibitem{ben12} Bensby, T., Feltzing, S., Gould, A., et al.: in Galactic Archaeology: Near-Field Cosmology and 
the Formation of the Milky Way, ASPC Vol. 458, p. 203 (2012) 
\bibitem{bi12} Bisterzo, S., Gallino, R., Straniero, O., Cristallo, S., K\"appeler, F.: MNRAS  \textbf{422}, 849 (2012) 
\bibitem{bo86} Boesgaard, A. M.,  Tripico, M. J.: ApJ \textbf{302}, L49 (1986) 
\bibitem{bo07} Boesgaard, A. M.: ApJ \textbf{667}, 1196 (2007)
\bibitem{bo88} Boffin, H.~M.~J.,  Jorissen, A.: A\&A \textbf{205}, 155 (1988)
\bibitem{bo94} Boffin, H. M. J.,  Za\'cs, L.: A\&A \textbf{291}, 811 (1994)
\bibitem{bo80} B\"ohm-Vitense, E.: ApJL, \textbf{239}, 79 (1980)
\bibitem{bo93} Bolte, M., Hesser, J.~E.,  Stetson, P.~B.: ApJL \textbf{408}, 89 (1993) 
\bibitem{bo44} Bondi, H,  Hoyle, F.: MNRAS  \textbf{104}, 273 (1944)
\bibitem{bo81} Bopp, B. W.,  Stencel, R. E.: ApJL \textbf{247}, 131 (1981)
\bibitem{br05} Bragaglia, A., et al.: in IAUS \textbf{228}, p. 243 (2005)
\bibitem{bro05} Brown, W. R. et al.: AJ \textbf{130}, 1097 (2005)
\bibitem{bu78} Buser, R.,  Kurucz, R. L.: A\&A \textbf{70}, 555 (1978)
\bibitem{bu83} Buzzoni, A., et al.: A\&A \textbf{128}, 94 (1983)
\bibitem{ca94} Carney et al.: AJ \textbf{107}, 2240 (1994)
\bibitem{ca01} Carney, B. W., et al.: AJ \textbf{122}, 3419 (2001)
\bibitem{ca05} Carney, B. W., Latham, D. W.,  Laird, J. B.: AJ \textbf{129}, 466 (2005)
\bibitem{ca09} Carretta, E., Bragaglia, A., Gratton, R.,  Lucatello, S.: A\&A \textbf{505}, 139 (2009)
\bibitem{ch09} Chen, X.,  Han, Z.: in IAUS \textbf{266}, p. 333 (2009)
\bibitem{cl11} Clarkson, W. I., et al.: ApJ \textbf{735}, 37 (2011)
\bibitem{cl02} Clewley, L., et al.: MNRAS  \textbf{337}, 87 (2002)
\bibitem{co12} Cohen, R. E.,  Sarajedini, A.: MNRAS  \textbf{419}, 342 (2012)
\bibitem{co96} C\^ot\'e, P., et al.: AJ \textbf{112}, 574 (1996)
\bibitem{da80} Davies, R. E.,  Pringle, J. E.: MNRAS  \textbf{191}, 599 (1980)
\bibitem{de97} Dearborn, D. S. P.,  Schramm, D. N.: Proc. Nat. Acad. Sci.\textbf{94}, 4836 (1997)
\bibitem{de06} De Marchi, F.: A\&A \textbf{459}, 489 (2006)
\bibitem{du91} Duquennoy, A.,  Mayor, M.: A\&A \textbf{248}, 485 (1991)
\bibitem{eg62} Eggen, O. J., Lynden-Bell, D.,  Sandage, A. R.: ApJ \textbf{136}, 748 (1962)
\bibitem{eg73} Eggleton, P. P.: MNRAS  \textbf{163}, 279 (1973)
\bibitem{fl94} Flynn, C., Sommer-Larsen, J.,  Christensen, P. R.: MNRAS  \textbf{267}, 77 (1994)
%\bibitem{fo11} For, B-Qing, Sneden, C.,  Preston, G.W.: ApJS  197, 29 (2011)
\bibitem{fu99} Fuhrmann, K.,  Bernkopf: A\&A \textbf{347}, 897 (1999)
\bibitem{fu11} Fuhrmann, K., et al.: MNRAS  \textbf{416}, 391 (2011) 
\bibitem{ge05} Geisler, D., et al.: AJ \textbf{129}, 1428 (2005)
\bibitem{gl94} Glaspey, J. W., Pritchet, C. J.,  Stetson, P. B.: AJ \textbf{108}, 271 (1994)
\bibitem{gl10} Glebbeek, E., et al.: in AIP Conf. Proc. 1314, p. 113 (2010)
\bibitem{gn97} Gnedin, O. Y.,  Ostriker, J. P. 1997: ApJ \textbf{474}, 223
\bibitem{gr87} Green, E. M., Demarque, P.,  King, C.: Revised Yale Isochrones and Luminosity Functions, Yale U. Press (1987)
\bibitem{ha95} Han, Z., et al.: MNRAS  \textbf{277}, 1443 (1995)
\bibitem{he77} Hesser, J. E., Hartwick, F. D. A.,  McClure, R. D.: ApJS  \textbf{33}, 471 (1977)
\bibitem{hi01} Hilditch, R. W.: An Introduction to Close Binary Stars, Cambridge Univ. Press (2001)
\bibitem{ho91} Hobbs, L. M.,  Mathieu, R. D.: PASP \textbf{103}, 431 (1991)
\bibitem{ho01} Horton, A. J., Bate, M. R.,  Bonnell, I. A.: MNRAS  \textbf{321}, 585 (2001)
\bibitem{in66} Innanen, K.: ApJ \textbf{143}, 153 (1966)
\bibitem{iv03} Ivans, I. I.: ApJ 592, 906 (2003)
\bibitem{jo00} Jorissen, A.,  van Eck, S., MmSAI \textbf{71}, 645 (2000)
\bibitem{ki66} King, I.: AJ \textbf{71}, 64 (1966)
\bibitem{ki94} Kinman, T. D., Suntzeff, N. B.,  Kraft, R. P.: AJ \textbf{108}, 1722 (1994) 
\bibitem{ki67} Kippenhahn, R,,  Weigert, A.: Z. Astrophys. \textbf{65}, 251 (1967)
\bibitem{ko55} Kopal, Z.: Ann. Astrophys.\textbf{18}, 379 (1955)
\bibitem{ko11} Koposov, S.~E., Gilmore, G., Walker, M.~G., et al.: ApJ \textbf{736}, 146 (2011) 
\bibitem{ku41} Kuiper, G. P.: ApJ \textbf{93}, 133 (1941)
\bibitem{la88a} Lance, C. M.: ApJS  \textbf{68}, 463 (1988a)
\bibitem{la88b} Lance, C. M.: ApJ \textbf{334}, 927 (1988b)
\bibitem{la02} Latham, D. W., et al.: AJ \textbf{124}, 1144 (2002)
\bibitem{le90} Lee, Y.-W.,  Demarque, P.: ApJS  \textbf{73}, 709 (1990)
\bibitem{le89} Leonard, P. J. T.: AJ \textbf{98}, 217 (1989)
\bibitem{li86a} Livio, M., et al.: MNRAS  \textbf{218}, 593 (1986a)
\bibitem{li86b} Livio, M., et al.: MNRAS  \textbf{222}, 235 (1986b)
\bibitem{ma78} Manduca, A.,  Bell, R. A.: ApJ \textbf{225}, 908 (1978)
\bibitem{ma97} Mandushev, G. I. et al.: AJ \textbf{114}, 1060 (1997)
\bibitem{ma09} Marino, A. F., et al.: A\&A \textbf{505}, 1099 (2009)
\bibitem{ma12} Marino, A. F., et al.: ApJ \textbf{746}, 14 (2012)
\bibitem{mas12} Masseron, T., Johnson, J.~A., Lucatello, S., et al.: ApJ \textbf{751}, 14 (2012) 
\bibitem{ma90} Mateo, M., et al.: AJ \textbf{100}, 469 (1990)
\bibitem{may96} Mayor, M., Duquennoy, A.,  Udry, S.: in ASPC Vol. 90, p. 190 (1996)
\bibitem{mc90} McClure, R. D.,  Woodsworth, A. W.: ApJ \textbf{352}, 709 (1990)
\bibitem{mc97} McClure, R. D.: PASP\textbf{109}, 536 (1997)
\bibitem{mc64} McCrea, W. H.: MNRAS  \textbf{128}, 147 (1964)
\bibitem{mcn97} McNamara, D. H.: PASP \textbf{109}, 1221 (1997)
\bibitem{me60} Melbourne, W. L.: ApJ \textbf{132}, 101 (1960) 
\bibitem{mi91} Michaud, G,  Charbonneau, P.: Sp. Sci. Rev. \textbf{57}, 1 (1991) 
\bibitem{mo04} Monelli, M., et al.: MmSAI \textbf{75}, 114 (2004)
\bibitem{mo00} Morrison, H., et al.: AJ \textbf{119}, 2254 (2000)
\bibitem{ne09} Newberg, H. J., Yanny, B.,  Willet, B. A.: ApJ \textbf{700}, L61 (2009)
\bibitem{no83} Norris, J.,  Freeman, K. C.: ApJ \textbf{266}, 130 (1983)
\bibitem{no97} Norris, J. E., Ryan, S. G.,  Beers, T. C.,  Deliyannis, C. P.: ApJ \textbf{485}, 370 (1997)
\bibitem{ol79} Olsen, E. H.: A\&AS \textbf{37}, 367 (1979)
\bibitem{ol80} Olsen, E. H.: A\&AS \textbf{39}, 205 (1980)
\bibitem{o60} Oort, J.: Bull. Astron. Inst, Neth. \textbf{15}, 45 (1960)
\bibitem{pa67} Paczynski, B.: in On the evolution of double stars, Obs. Royal Belgique, Communications, Serie B, No. 17, p. 122 (1967)
\bibitem{pa07} Paczynski, B. Sienkiewicz,  Szczyiel, D. M.: MNRAS  \textbf{378}, 961 (2007)  
\bibitem{pa00} Pamyatnikh, A. A.: in ASPC Vol. 210, p. 215 (2000)
\bibitem{pe69} Perry, C. L.: AJ \textbf{74}, 139 (1969)
\bibitem{pe99} Petersen, J. O.,  Christensen-Dalsgaard, J.: A\&A \textbf{352}, 547 (1999)
\bibitem{ph68} Philip, A. G. D.,  Sanduleak, N.: Bol. Obs. Tonanzintla y Tacubaya \textbf{4}, 253 (1968)
\bibitem{pi83} Pier, J. R.: ApJS  \textbf{53}, 791 (1983)
\bibitem{pi12} Pietrzy{\'n}ski, G., Thompson, I.~B., Gieren, W., et al.: Nature \textbf{484}, 75 (2012) 
\bibitem{pi99} Pinsonneault, M. H., et al.: ApJ \textbf{527}, 180 (1999)
\bibitem{pi01} Pinsonneault, M. H., DePoy, D. L.,  Coffee, M.: ApJ \textbf{556}, L59 (2001)
\bibitem{pi02} Pinsonneault, M. H., et al.: ApJ \textbf{574}, 398 (2002)
\bibitem{pi04} Piotto, G., et al.: ApJ \textbf{604}, L109 (2004)
\bibitem{po08} Poretti, E., et al.: ApJ \textbf{685}, 947 (2008)
\bibitem{pre91} Preston, G. W., Shectman, S. A.,  Beers, T. C.: ApJS  \textbf{76}, 1001 (1991)
\bibitem{pre94a} Preston, G. W.: AJ \textbf{108}, 2267 (1994a)
\bibitem{pre94b} Preston, G. W., Beers, T. C.,  Shectman, S. A.: AJ \textbf{108}, 538 (1994b)
\bibitem{pre98} Preston, G. W.,  Landolt, A. U.: AJ \textbf{115}, 2515 (1998)
\bibitem{pre99} Preston, G. W.,  Landolt, A. U.: AJ \textbf{118}, 3006 (1999)
\bibitem{pre00} Preston, G. W.,  Sneden, C.: AJ \textbf{120}, 1014 (2000; PS00)
\bibitem{pre06} Preston, G. W., et al.: AJ \textbf{132}, 1714 (2006)
\bibitem{pre09} Preston, G. W.: PASA \textbf{26}, 372 (2009)
\bibitem{pre11} Preston, G. W.: AJ \textbf{141}, 6 (2011)
\bibitem{pr91} Pritchet, C. J.,  Glaspey, J. W.: ApJ \textbf{373}, 105 (1991)
\bibitem{ro71} Rodgers, A. W.: ApJ \textbf{165}, 581 (1971) 
\bibitem{ro83} Rodgers, A. W, Harding, P.,  Sadler, E.: ApJ \textbf{244}, 912 (1983)
\bibitem{ry01} Ryan, S. G. et al.: ApJ \textbf{547}, 231 (2001)
\bibitem{ry02} Ryan, S. G. et al.: ApJ \textbf{571}, 501 (2002)
\bibitem{sa78} Sahade, J.,  Wood, F. B.: in Interacting Binary Stars, Pergamon Press, p. 1 (1978)
\bibitem{sa53} Sandage, A. R.: AJ \textbf{58}, 61 (1953)
\bibitem{sa87} Sandage, A. R.: AJ \textbf{93}, 610 (1987)
%\bibitem{sa06} Sandage, A. R. 2006: AJ 131, 1750
\bibitem{sa88} Sanduleak, N.: ApJS  \textbf{66}, 309 (1988)
\bibitem{sa93} Sarajedini, A.: in ASPC Vol. 53, 14 (1993)
\bibitem{se66} Searle, L.,  Rodgers, A. W.: ApJ \textbf{143}, 809 (1966)
\bibitem{se07} Sepinsky, J. F., et al.: ApJ \textbf{667}, 1170 (2007)
\bibitem{se09} Sepinsky, J. F., et al.: ApJ \textbf{702}, 1387 (2009)
\bibitem{se10} Sepinsky, J. F., et al.: ApJ \textbf{724}, 546 (2010) 
\bibitem{se68} S\'ersic, J. L.: Atlas de galaxias australes, Cordoba, Obs. Astronomico (1968)
\bibitem{sh01} Shetrone, M. D., C\^ot\'e, P.,  Sargent, W. L. W.: ApJ \textbf{548}, 592 (2001)
\bibitem{sh03} Shetrone, M, et al.: AJ \textbf{125}, 684 (2003)
\bibitem{si04} Sirko, E., et al.: AJ \textbf{127}, 899 (2004)
\bibitem{sm94} Smecker-Hane, T.~A., Stetson, P.~B., Hesser, J.~E.,  Lehnert, M.~D.\: AJ \textbf{108}, 507 (1994) 
\bibitem{so04} Soker, N.: MNRAS  \textbf{350}, 1366 (2004)
\bibitem{so11} Soszy\'nski, I, et al.: Acta Astron. \textbf{61}, 1 (2011)
\bibitem{sp82} Spite, F.,  Spite, M.: A\&A \textbf{115}, 357 (1982)
\bibitem{sp00} Spite, M. et al.: A\&A \textbf{360}, 1077 (2000)
\bibitem{st07} Stancliffe, R. J., et al.: A\&A  \textbf{464}, L57 (2007)
\bibitem{st10} Stancliffe, R. J.: MmSAI \textbf{81}, 1064 (2010)
\bibitem{st91} Stetson, P. B.: AJ \textbf{102}, 589 (1991)
\bibitem{st41} Struve, O.: ApJ \textbf{93}, 104 (1941)
\bibitem{th96} Theuns, T., Boffin, H. M. J.,  Jorissen, A.: MNRAS  \textbf{280}, 1264 (1996)
\bibitem{th08} Thompson, I. B., et al.: ApJ \textbf{677}, 556 (2008)
\bibitem{th92} Thorburn, J. A.,  Beers, T. C.: BAAS \textbf{24}, 1278 (1992)
\bibitem{th94} Thorburn, J. A.: ApJ \textbf{421}, 318 (1994)
\bibitem{ti06} Tian, B., et al.: A\&A \textbf{455}, 247 (2006)
\bibitem{to06} Tokovinin, A., et al.: A\&A \textbf{450}, 681 (2006)
\bibitem{un96} Univane, M, Wyse, R. F. G.,  Gilmore, G.: MNRAS  \textbf{278}, 727 (1996)
\bibitem{va03} VandenBergh, D. A.,  Clem, J. L.: AJ \textbf{126}, 778 (2003)
\bibitem{va10} VandenBergh, D. A., Casagrande, L.,  Stetson, P. B.: AJ \textbf{140}, 1020 (2010)
\bibitem{va94} Vanture, A. D., Wallerstein, G.,  Brown, J. A.: PASP \textbf{106}, 835 (1994)
\bibitem{va04} Vauclair, S.: ApJ \textbf{605}, 874 (2004)
\bibitem{ve04} Venn, K. A.: AJ \textbf{128}, 1177 (2004)
\bibitem{wa60} Wallerstein, G.  Carlsoln, M.: ApJ \textbf{132}, 276 (1960)
\bibitem{wi62} Wildey, et al., et al.: ApJ \textbf{135}, 94 (1962)
\bibitem{wi99a} Wilhelm, R., et al.: AJ 117, 2308 (1999a)
\bibitem{wi99b} Wilhelm, R., et al.: AJ 117, 2329 (1999b)
\bibitem{xu11} Xue, X.-X., et al.: ApJ \textbf{738}, 79 (2011)
\bibitem{ya00} Yanny, B., et al.: ApJ \textbf{540}, 825 (2000)
\bibitem{yi01} Yi, S., et al.: ApJS  \textbf{136}, 417 (2001)
\bibitem{zo00} Zoccali, M., et al.: ApJ \textbf{538}, 239 (2000)
\end{thebibliography}


==> refsills.tex <==
\begin{thebibliography}{99}

\bibitem{Aarseth12} Aarseth, S.~J.: MNRAS {\bf  422}, 841  (2012)

\bibitem{BailynPinsonneault95} Bailyn, C.~D., Pinsonneault, M.~H.: ApJ {\bf  439}, 705  (1995)

\bibitem{Belczynski08} Belczynski, K., Kalogera, V., Rasio, F.~A., et al.:
%Taam R.~E., 
%Zezas A., Bulik T., Maccarone T.~J., Ivanova N.: 
ApJS {\bf  174}, 223 (2008)

\bibitem{BenzHills87} Benz, W., Hills, J.~G.: ApJ {\bf  323}, 614  (1987)

\bibitem{Chatterjee10} Chatterjee, S., Fregeau, J.~M., Umbreit, S., Rasio, F.~A.: ApJ {\bf  719}, 915  (2010)

\bibitem{ChenHan04} Chen, X., Han, Z.: MNRAS {\bf  355}, 1182  (2004)

\bibitem{ChenHan07} Chen, X., Han, Z.: in Unsolved Problems in Stellar Physics, AIPC Vol. 948, p. 431 (2007)

\bibitem{ChenHan08} Chen, X., Han, Z.: MNRAS {\bf  384}, 1263  (2008a)

\bibitem{ChenHan08b} Chen, X., Han, Z.: MNRAS {\bf  387}, 1416 (2008b)

\bibitem{Cohen12} Cohen, R.~E., Sarajedini, A.: MNRAS {\bf  419}, 342 (2012)

\bibitem{DAntona05} D'Antona, F., Bellazzini, M., Caloi, V., Pecci, F.~F., Galleti, S., Rood, R.~T.: ApJ {\bf  631}, 868 (2005)

\bibitem{MMAMS} Gaburov, E., Lombardi, J.~C., Portegies Zwart, S.: MNRAS {\bf  383}, L5 (2008)

\bibitem{Glebbeek08a} Glebbeek, E., Pols, O.~R., Hurley, J.~R.: A\&A {\bf  488}, 1007 (2008)

\bibitem{Glebbeek08b} Glebbeek, E., Pols, O.~R.: A\&A {\bf  488}, 1017 (2008)

\bibitem{GlebbeekSills10} Glebbeek, E., Sills, A., Leigh, N.: MNRAS {\bf  408}, 1267 (2010)

\bibitem{Glebbeek10} Glebbeek, E., Sills, A., Hu, H., Stancliffe, R.~J.: in AIPC Vol. 1314, p. 113 (2010)

\bibitem{Hills80} Hills, J.~G.: ApJ {\bf  235}, 986 (1980)

\bibitem{Hurley02} Hurley, J.~R., Tout, C.~A., Pols, O.~R.: MNRAS {\bf  329}, 897 (2002)

\bibitem{Hypki13} Hypki, A., Giersz, M.: MNRAS {\bf  429}, 1221 (2013)

\bibitem{Ivanova05} Ivanova, N., Belczynski, K., Fregeau, J.~M., Rasio, F.~A.: MNRAS {\bf  358}, 572 (2005)

\bibitem{Ivanova13} Ivanova, N., et al.: A\&ARv, 21, 59 (2013)

\bibitem{Kawaler88} Kawaler, S.~D.: ApJ {\bf  333}, 236 (1988)

\bibitem{Kipp67} Kippenhahn, R., Weigert, A.: Zeitschrift Astron. {\bf 65}, 251 (1967)

\bibitem{lau70}
{Lauterborn}, D.: A\&A \textbf{7}, 150 (1970)

\bibitem{Leonard89} Leonard, P.~J.~T.: AJ {\bf  98}, 217 (1989)

\bibitem{LeonardLivio95} Leonard, P.~J.~T., Livio, M.: ApJL {\bf  447}, 121 (1995)

\bibitem{Lombardi95} Lombardi, J. C., Jr., Rasio, F.~A., Shapiro, S.~L.  : ApJL {\bf  445}, 117 (1995)

\bibitem{Lombardi96} Lombardi, J.~C., Jr., Rasio, F.~A., Shapiro, S.~L.: ApJ {\bf  468}, 797 (1996)

\bibitem{MMAS} Lombardi, J.~C., Jr., Warren, J.~S., Rasio, F.~A., Sills, A., Warren, A.~R.: ApJ {\bf  568}, 939 (2002)

\bibitem{Lu10} Lu, P., Deng, L.~C., Zhang, X.~B.: MNRAS {\bf  409}, 1013 (2010)

\bibitem{Maeder13} Maeder, A., Meynet, G., Lagarde, N., Charbonnel, C.: A\&A {\bf 553}, A1 (2013)

\bibitem{MattPudritz05} Matt, S., Pudritz, R.~E.: ApJ {\bf  632}, L135 (2005)

\bibitem{Nelson01} Nelson, C.~A., Eggleton, P.~P.: ApJ {\bf  552}, 664 (2001)

\bibitem{Ouellette98} Ouellette, J.~A., Pritchet, C.~J.: AJ {\bf  115}, 2539 (1998)

\bibitem{SPZ96} Portegies Zwart, S.~F., Verbunt, F.: A\&A {\bf  309}, 179 (1996)

\bibitem{SPZ13} Portegies Zwart, S., McMillan, S.~L.~W., van Elteren, E., Pelupessy, I., de Vries, N.: CoPhC {\bf 183}, 456 (2013)

\bibitem{Procter95} Procter Sills, A., Bailyn, C.~D., Demarque, P.: ApJ {\bf  455}, L163 (1995)

\bibitem{Sandquist97} Sandquist, E.~L., Bolte, M., Hernquist, L.: ApJ {\bf  477}, 335 (1997)

\bibitem{Santolamazza01} Santolamazza, P., Marconi, M., Bono, G., Caputo, F., Cassisi, S., Gilliland, R.~L.: ApJ {\bf  554}, 1124 (2001)

\bibitem{SillsLombardi97} Sills, A., Lombardi, J.~C., Jr.: ApJ {\bf  484}, L51 (1997)

\bibitem{Sills97} Sills, A., Lombardi, J.~C., Jr., Bailyn, C.~D., Demarque, P., Rasio F.~A., Shapiro S.~L.: ApJ {\bf  487}, 290 (1997)

\bibitem{Sills01} Sills, A., Faber, J.~A., Lombardi, J.~C., Jr., Rasio, F.~A., Warren, A.~R.: ApJ {\bf  548}, 323 (2001)

\bibitem{Sills05} Sills, A., Adams, T., Davies, M.~B.: MNRAS {\bf  358}, 716 (2005)

\bibitem{Sills09} Sills, A., Karakas, A., Lattanzio, J.: ApJ {\bf  692}, 1411 (2009)

\bibitem{Sills13} Sills A., Glebbeek, E., Chatterjee, S., Rasio, F.~A.: ApJ {\bf 777}, 105  (2013)

\bibitem{Templeton02} Templeton, M., Basu, S., Demarque, P.: ApJ {\bf  576}, 963 (2002)

\bibitem{Tian06} Tian, B., Deng, L., Han, Z., Zhang, X.~B.: A\&A {\bf  455}, 247 (2006)

\end{thebibliography}

